Jenga: Effective Memory Management for Serving LLM with Heterogeneity

Large language models (LLMs) are widely used but expensive to run, especially as inference workloads grow. To lower costs, maximizing the request batch size by managing GPU memory efficiently is crucial. While PagedAttention has recently been proposed to improve the efficiency of memory management, we find that the growing heterogeneity in the embeddings dimensions, attention, and access patterns of modern LLM architectures introduces new challenges for memory allocation. In this paper, we present Jenga, a novel memory allocation framework for heterogeneous embeddings in LLMs. Jenga tackles two key challenges: (1) minimizing memory fragmentation when managing embeddings of different sizes, and (2) enabling flexible caching and eviction policies tailored to the specific token-dependency patterns of various layers. Jenga employs a two-level memory allocator, leveraging the least common multiple (LCM) of embedding sizes to optimize memory usage and providing APIs to express layer-specific caching logic to enhance memory reuse. We implemente Jenga on vLLM, a state-of-the-art LLM inference engine, and evaluate it with diverse LLMs, datasets, and GPU configurations. Evaluations show that Jenga improves GPU memory utilization by up to 79.6%, and increases serving throughput by up to 4.92x (1.80x on average).

==> impl.tex <==
\tightsection{Implementation}
\begin{figure}[t]
    \centering
    \small
\begin{minted}{python}
def custom_kv_cache_for_gemma2(config):
 custom_layers = {}
 sliding_window, hidden_size = config.get_model_info()
 for i in range(config.num_layers):
  if i % 2 == 0:
   custom_layers[i] = SlidingWindowLayer(sliding_window, hidden_size)
  else:
   custom_layers[i] = SelfAttentionLayer(hidden_size)
 return custom_layers
\end{minted}
    \vspace{-1em}
    \caption{Define \gemma structure for \sys, whose odd layers are self-attention and even layers are sliding window}
    \label{fig:sys-gemma}
\end{figure}
\sys is implemented with about 4000 lines of Python code on top of vLLM and does not require any change of CUDA kernels. \sys is compatible with all the 90 models in \latestvllm. %, the latest release when the paper was submitted on Dec 10th. \shu{I don't think the last half sentence is needed..}


\sys is transparent to users of the inference engine. Model vendors only need to declare the layer type explicitly, as shown in \Cref{fig:sys-gemma}. All memory management decisions can be performed automatically by \sys. \zcsay{implementation section is too short. Recover the previous 6.1?}



% \subsection{Model execution with the Page-layer Partition Layout}
% \label{sec:custom_id}

% As mentioned in \Cref{sec:new-layout}, \sys uses a slightly different memory layout than standard PagedAttention to enable page sharing between different types. In this section, we will provide more details on how to represent the allocated memory to make the layout compatible with current PagedAttention kernels.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/exec_start_ptr.pdf}
%     \caption{\texttt{kv\_cache\_start\_ptr}}
%     \label{fig:exec_start_ptr}
% \end{figure}

% The allocated memory for a layer can be fully represented with the following variables, which are the input to the PagedAttention kernel.
% \begin{itemize}
%     \item \texttt{kv\_cache\_start\_ptr}: The start pointer of the KV cache tensor (\Cref{fig:exec_start_ptr}). It points to the start of each layer in the first small page (P0). Due to the different pointers of layers in the same type, they can use different memory spaces with the same page ID.
%     \item \texttt{pageid\_exec}: the page ID passed to the \texttt{block\_table} parameter of paged attention kernels, which is calcuated by $pageid\_exec = pageid\_alloc * num\_layer\_this\_type$. For example, small pages $[0,2,6,7]$ are allocated for the four image tokens in \Cref{fig:exec_cross_1}, and there are 2 cross-attention layers that need image token KV cache, so \texttt{pageid\_exec} of layer \texttt{cross.1} becomes $[0,4,12,14]$. The \texttt{pageid\_exec}  of all layers in \Cref{fig:two_level_overview} are shown in \Cref{tab:pageid_exec}.
%     \item \texttt{page\_size\_exec}: the page size of each layer, defined by $\text{tokens\_per\_page} \times \text{kv\_hidden\_size}$, and with the property $\text{page\_size\_exec} \times \text{num\_layer\_this\_type} = \text{small\_page\_size}$. % The \texttt{page\_size\_exec} is equal to the page size of PagedAttention. 
% \end{itemize}


% \begin{table}[t]
%     \centering
%     \begin{tabular}{ccc}
%     \toprule
%          \textbf{\texttt{layer\_id}} & \textbf{\texttt{pageid\_alloc} }& \textbf{\texttt{pageid\_exec}}  \\
%     \midrule
%        cross.0, cross.1  & 0, 2, 6, 7 & 0, 4, 12, 14 \\
%        self.0, self.1, self.2 & 2, 3 & 6, 9 \\
%      \bottomrule
%     \end{tabular}
%     \caption{mapping of \texttt{pageid\_alloc} and \texttt{pageid\_exec}}
%     \label{tab:pageid_exec}
% \end{table}

% Another choice for supporting \sys's layout is to give the same \texttt{KV\_cache\_start\_ptr} and different \texttt{pageid\_exec} to different layers of the same type. It also does not need to change the attention kernels, but the inference engine workers need to prepare different attention metadata for each layer, which can introduce a large runtime overhead. Therefore, \sys does not take this option.



==> intro.tex <==
\section{Introduction}
\zcsay{extended from Ion's outline (in memory management google doc):)}
\begin{itemize}
\item LLM inference workload are memory-bound.
\item Challenge: 
\item{\kt{Kuntai Rewrite start}}
\item{LLM inference workload are quickly growing, and the LLM inference is in general bounded by memory capacity.}
\item{sdfasdf}
\item{To alleviate GPU memory pressure, more and more LLMs choose to substitute memory-consuming self-attention to \textit{\textbf{mixing}} different types of attention mechanisms in the same model to handle long context while controlling the size of KV caches (sliding window + self attention), or to handle different types of modalities (self attention + cross attention).}
\item{Such trend creates new challenges to the memory allocator, as the \textit{\textbf{tensor shape}} and the \textit{\textbf{memory allocation pattern}} are no longer aligned across layers since different layers may use different attention mechanisms.}
\item{Existing solutions fall short when handling such mix-attention models.}
\item{Previous work 1: GPU memory virtualization, where the hardware allows a large KV cache tensor to be stored into non-contiguous small pages, but \zc{large malloc overhead, very bad for small models; cross platform support}}
\item{Previous work 1: PagedAttention, which assumes the memory allocation patterns and the tensor shapes of KV caches are aligned across layers and manage the KV caches on top of this assumption. Advantage: no memory waste when the LLM models only use one types of attention layers across model. Disadvantage: high amount of memory waste when re-purposing it to those models with different types of attentions.}
\item{Previous work 2: Fix-ratio allcoation (for each types of attention layers, allocate a fixed-size memory pool for its KV cache). This performs well when the size of different types of KV cache size for different layers has a fixed ratio (e.g. }
\item{\kt{Kuntai rewrite end}}
\zc{This intro flow only focus on allocation, but prefix caching is also a large part. Should we position prefix caching as a new challenge of the proposed new allocator?}
\item Inference workloads are growing (maybe give some data that for many users, inference workloads dominate training workloads; probably even for frontier labs, let alone the others)
% \kt{The sentence is probably a bit too true to feel like i an argument. A possible alternative: LLM inference systems are serving more and more heterogeneous models.}
\item Despite the increase in the GPU memory over the past 2 years, many inference workloads are still memory bounded \zc{will highlight capacity bound}
% \kt{After re-read this, this sentence is not spelling out an issue that directly connects to the end-to-end metrics}
% \kt{Also I heard that the total capacity of HBM manufacturing is bounded, that's probably the main reason of GPU mem}
\begin{itemize}
    \item Longer contexts
    \item MoE model (lower compute density) (\zcsay{we will cover jamba and hunyuan, though no optimization on MoE layer, we can get speedup from larger batch size})
    \item Large models, e.g., Llama 3 405B
\end{itemize}

\item PagedAttention was introduced to address the memory bottleneck by increasing the efficiency of memory allocation, which led to higher throughput and lower costs.
However, this is no longer enough. Can cite the 78\% memory waste example of mllama.
\item Why?: Key assumption of PagedAttention: all tokens have the same KV cache size. No longer hold for new models \kt{This sentence is pointing out the phenomena (different tokens have different KV cache sizes) but does not provide a rationale behind it. An example: The key assumption behind PagedAttention is that the attention layers are \textbf{\textit{ homogeneous}} inside the same model, and thus the KV caches has the same shape across different tokens and different layers. However, as more and more techniques are introduced to reduce the KV cache sizes (e.g. sliding window attention, token dropping), or to incorporate with different modalities (e.g. cross attention), the attention layers are becoming more and more \textbf{\textit{heterogeneous}} even inside the same model, resulting in different KV cache sizes for different tokens and layers.} \sout{Models are becoming more complex}  \zc{updated} (e.g.:
    \begin{itemize}
        \item multi-modality, different modality may have different number of tokens (mllama, NVLM, flamingo)
        \item scalable attention techniques like sliding window attention, token drop, \sout{kv cache sharing}
        \item serving multiple models together (e.g., speculative decoding, LORAs)
    \end{itemize}
\item As a result, they require different page sizes, which is a challenge for most memory allocation system
\item Opportunity: page size are highly aligned ($m\times 2^n$) \kt{There is no direct logic connection between $m\times 2^n$ and we can have practical benefit}, number of different page size is limited. Which is not held in traditional OS memory management
\item Main idea: two-level allocation, level0 as the lcm of all page size, and some more details. Highlight this is different from OS memory allocation 
\item Problems
    \begin{itemize}
        \item Memory allocation: how to avoid internal fragmentation in level0 page
        \item Accelerators like GPUs needs regular pages (with only one page size) to execute efficiently
        \item Cache replacement policies. 1. better cache replacement policies for single type (e.g., for sliding window-based attention) 2. fair replacement policies for different types
    \end{itemize}
\item Solutions
    \begin{itemize}
        \item Memory allocation: request-aware allocation
        \item Execution: represent the allocation result as normal pages, with minimal changes to the workers
        \item Cache replace policy: flexible interface to custom last access time of different types of pages, two-level LRU for fair replacement
    \end{itemize}
\item Evaluation shows that xxxx
\item Contributions: xxx

page size is not the key problem
how allocate, how use(todo refine, shared kv), how drop it
% and 
% Solution:
% multiple page sizes
% Problem: how do you do it so you can limit fragmentation and don’t hurt performance (i.e., access times). 
% Solution: 
% Two-level…

% Somewhere we need to emphasize this is a new memory organization not used before in OSes.

\end{itemize}

% \zcsay{
% heterogeneous -> token have different types of memory and shapes. \\
% different shape -> allocation fragmentation \\
% different type -> different hit rule \& fair prefix caching


% problem: all three types of work cannot do allocation. Not list related work on prefix caching
% }

% \zcsay{
% we need to design a new memory allocator. 
% It has new challenge in prefix caching.
% Problem: not our sys cause challenge in prefix caching, but heterogeneous
% }

0. LLM is popular.

1. LLM inference workload is getting larger. Key: \zcsay{previous work shows that large number of request is important for throughput}. Main challenge: how to fit maximum number of requests into into GPU memory, 

2. Evolving many new techniques; Trend: LLMs are becoming heterogeneous. Concretely, they re-purpose attention layers for different purposes, e.g. handling different modalities (e.g. cross-attention), or controlling KV caches sizes (sliding window), or representing all historical information into a very large but fixed size of tensor (e.g. mamba)

3. Unique opportunity: different attention layers in the models allocates KV caches with different shapes and for different tokens.

4. Challenge: how to design an memory allocator in LLM inference engines that can allocate different shapes of tensors for different tokens, to fit as many requests into GPU memory as possible?

4. Previous work
 4.1: PagedAttention: memory allocator agnostic to different layers --> large memory waste
 4.2: vAttention: 
 use a fixed size (64KB) as the minimum allocation granularity, not suitable for those small models. Use a smaller size --> significantly increase allocation overhead. \zcsay{not cross platform}
 4.3: A practical baseline: fix-ratio allocation. Large memory waste. \todo{evaluation on fix-size allocation?}
 

6. Why previous work is insufficient: all approaches partition the whole memory space into pre-defined static pieces (fixed-size pages in Paged Attention and vAttention, fixed ratio in fixed size partition), but the optimal KV cache size partition for different attention layers hugely depends on the context length, and thus vary a lot between different batches.

7. We argue that: we need to allow the memory allocator to dynamically adapt its memory partition strategy, based on the size of KV caches generated by different types of attention layers \textit{inside the current batch}

8. Insight: empirically, though different models have highly heterogeneous attention layers, the heterogeneity inside the same model is limited. Concretely, there are at most 5 different types of KV cache allocation granularity, and they are typically a multiplier of $2^10$ (for the sake of computation efficiency).
As a result, we can create a \textit{compatibility layer}, which can be repurposed for different types of KV cache allocation granularity, and then allocate different types of KV caches on top of such \textit{comaptibility layer}.


9. A strawmen design: GCD as the compatibility layer. Needs to change the API of other parts in inference engine (e.g. different kernels for different hardwares) to incorporate a wide range of potential GCDs, introducing large engineering, deployment and performance overhead.


10. Our solution: LCM as the compatibility layer. Can reuse existing API of other parts in inference engines. 

11. To make this solution practical, we also need to handle prefix caching.

12. Our evaluation shows that xxx

13. To summarize, our contributions are:
    13.A. A memory allocator that minimizes GPU memory fragmentation across different types of layers.
    13.B. Prefix caching
    13.C. Implementation on top of production-level inference engine.
    13.D. xxx memory saving and xxx speedup

% 8. Insight: empirically, in order to be hardware-compute-friendly, the KV cache size allocation granularity are pre-determined, limited number of types, and  before runtime, and between different layers simultaneously have a very large GCD (2^10) and a relatively small LCM (<10x GCD). 


% 7. However, all possible types of memory are pre-known and the number is limited, so we can partition the memory that compatible to all types, and further partition it as needed. Specifically, LCM, ..., 

% LCM: not need to change kernel

% LCM good: small size is not bottlenecck, allow small fragementation


% Why previous work is not enough: the size ratio between different attention layer's KV caches can be hugely different between requests, but the allocated KV cache space ratio for different attention layers are the same.



% 6. Our insight: previous work has a static mapping between tensor tokens and KV cache addresses

% 6. Our insight: previous work cannot repurposed the same memory for different tokens with different shapes.

% 6. Our insight: the allocation of previous work are fine-grained on tokens but coarse-grained on model layers -- it allocates KV caches for all layers simultaneously

% 6. Our insight: previous work lacks the ability of allocating different size of memory (not fundamental enough)-> due to xxx  LLM's special property, we can do it by xxx.

% 6. all appoaches somehow introduce a fix size, lacks flexibility for allocate different size memory

% 6. All approaches partition the whole memory space into pre-defined static pieces (fixed-size pages in Paged Attention and vAttention, fixed ratio in fixed size partition), and cannot handle the dynamic scenarios where both the size of each components and the memory size ratio of different types of memory are changing.


% Our insight: previous work 


% Goal: we aim to design a memory allocator in LLM inference engines that can serve heterogeneous models with low memory fragmentation.
% \zcsay{then you need to prove we are compatible with ALL inference engine features}

% \kt{
% Flow 2: we aim to design an in-GPU KV cache caching system for heterogeneous models. Challenge:
% 1. cache tensors with different shapes while maximizing memory efficiency
% 2. eviction
% }

==> intro_v2.tex <==
\section{Introduction}

{Ion's Proposed Flow:
\begin{itemize}
\item LLMs are changing the world.
\item LLM inference is growing in importance due to the generality of LLMs (i.e., you don't need to train them for each task) and test-time inference/compute.
\item LLM inference is hugely expensive; making it efficient is the key.
\item (Remind people how did we get to vLLM) Token generation is sequential $\rightarrow$ batches to improve parallelism but memory becomes a bottleneck $\rightarrow$ page attention to improve memory utilization and increase batch size.
\item Many things have changed since PagedAttention has been introduced (e.g., multi-modal models, mixed state-space, etc) $\rightarrow$ The result: we need to support multiple embedding sizes. 
\item So key challenge is to support multiple embedding sizes and maximize mem utilization. One solution is to have larger page sizes but can lead to internal fragmentation.  
\item Our solution: two-level memory management based on LCM.
\item Also heterogeneity brings new (fundamental) challenges to how we do eviction, caching.
\item ...
\end{itemize}
}

\subsection{Kuntai's version}
\woosuk{I think the current flow has too many hops. Why don't we start from directly pointing out the difficulty of managing heterogeneous memory states?
Also, I think we should not focus too much on fragmentation and memory waste, since it does not include prefix caching for heterogeneous layers.}

Large language models (LLMs) are becoming more and more popular. Billions of people use ChatGPT~\tocite{}, and millions of people use Github Copilot to write code and documentations~\tocite{}.
To handle huge LLM workload, people find that it is crucial to enlarge LLM inference \textit{batch size}, which allows more requests to be processed within single LLM forwarding pass while only marginally increase the LLM forwarding latency~\tocite{}. \zhuohan{Why talk about batch size here? I feel the concept of batch size comes out of the blue and seems unnecessary here.} \zcsay{we need to point out why avoiding memory waste is important}
% without  is to perform LLM inference with as large batch size as possible, so that 
% maximally enlarge the LLM inference batch size, by designing a GPU memory allocator that can fit as many requests into the GPU memory as the GPU memory permits.
Based on such insight, people develop LLM inference engines (e.g., vLLM~\tocite{} and TGI~\tocite{}) that maximally increase the batch size (by using customized GPU memory allocator to fit as many requests into GPU memory as possible) and thus serve LLM inference requests with much high throughput without inflating the end-to-end latency.

% \zcsay{We need to highlight batch size is important here, instead of saying "they have good batch size".}
% \kt{My feeling is that we need to spend a lot of text in intro if we want to explain why large batch size leads to higher throughput (and this text does not really push the logic forward). }
% Let me try: Due to the xxx property of LLM serving, the throughput of these inference engines highly depends on the number of LLM inference requests that can be batched together, so they design memory allocators to maximally batches as many LLM inference requests as the GPU memory permits}


Alongside the significant rise of LLM inference workloads, LLM architectures also get increasingly \textit{heterogeneous}, where LLMs use traditional attention layers \textbf{\textit{together with}} other types of attention layer to better customize the model for specific user needs, while maximally preserving the accuracy of the models. 
For example, \llama 3.2~\cite{dubey2024llama} leverages cross-attention layers for image tokens to handle multi-modality inputs; \gemma~\cite{team2024gemma} leverages sliding window attention layer to better control the KV cache sizes when handling long input context.
% , or representing all historical information into a very large but fixed size of tensor (e.g. mamba)
Such heterogeneous attention layers also generate KV caches (the intermediate data of attention layers that need to be cached to generate new tokens) with \textit{different KV cache granularities} (we define the KV cache granularity as the KV cache size for one single token) and \textit{for different sets of tokens}.

% For example, \llama 3.2 generates KV cache for image tokens and text tokens seperately, where the KV cache granularity for each text token is $4\times$ larger than that of image tokens. 

As a result, the research question of this paper is: How to design a GPU memory allocator for LLM inference engines that allows maximum batch size for heterogeneous LLM architectures by allocating KV caches with minimum GPU memory fragmentation?

% There are three types of prior work that handles this challenge, but they all introduces significant memory waste. \zcsay{Related work part is a little long, is it possible to only discuss paged attention here, and put other parts in a seperate discussion section?}

Existing inference engines tackle this research question by PagedAttention.
The key innovations of PagedAttention is that it allows partitioning the KV caches generated by LLMs along token dimensions and store each piece of partitioned KV cache into non-adjacent GPU memory addresses, with minimum impact on LLM inference performance.
% Concretely, it calculates the amount of GPU memory consumed by LLM when handling a fixed amount of tokens (by default 16 in vLLM), and then partitions the GPU memory into pages using such value.
Such PagedAttention-based inference engines has very low GPU memory fragmentation when handling those models that only uses one type of attention layers.
However, PagedAttention has significant GPU memory fragmentation when supporting LLMs that use different types of attention layers.
Concretely \kt{Quantify the amount of memory waste here} %\zcsay{TODO: show the memory waste calculated in sec 3}.

The key reason behind such GPU memory fragmentation is that PagedAttention's GPU memory allocation strategy is \textit{agnostic} to different types of attention layers, resulting in fixed GPU memory allocation ratio between different attention layer types.
However, the ratio between the actual GPU memory required by the KV cache of different attention layer types \textit{hugely varies} between different batches.
\kt{Quantify how much such allocation ratio can vary.}
As a result, the GPU memory fragmentation can be substantial when the fixed allocation ratio significantly mismatches the actual ratio for the current batch.

% approaches shares the same limitation: they all partition the whole memory space into pre-defined static pieces (fixed-size pages in Paged Attention and vAttention, fixed ratio in fixed size partition), but the optimal KV cache size partition for different attention layers hugely depends on the context length, and thus vary a lot between different batches.

% The second type of work is vAttention that allows the LLM applications to allocate large tensors, while the under GPU driver partitions the tensor into small pages (each page is of size 64KB) and performs memory allocation based on such small pages. 
% This design offloads the memory allocation complexity to GPU drivers, which introduces much higher engineering overhead compared to performing memory allocation inside LLM serving engines, as GPU drivers are much difficult to program, and the effort of changing the driver cannot be reused by other types of GPUs. \zcsay{not true, discussion needed}

% The third type of work is creating a fix-size memory pool for different types of KV caches, and then perform memory allocation inside each pool. 
% As a result, the GPU memory allocation ratio between different types of attention layers are fixed, and result in high memory waste when serving models with different types of attentions.

We argue that: instead of fixing the ratio of GPU memory size between different types of attention layers, the memory allocator needs to be able to \textbf{\textit{dynamically}} adjust such ratio to match the actual GPU memory requirement ratio of the current LLM inference batch.

Such dynamic memory allocation is in general difficult and motivates decades of research~\tocite{}.
However, in LLM applications, such problem is much simpler to tackle: though different LLMs have highly heterogeneous attention layers, empirically we observe that the heterogeneity inside the same LLM is much more \textbf{\textit{limited}}. 
Concretely, a typical LLM uses at most 3 different types of attention layers, and the size of those KV caches are typically a multiplier of $2^{10}$ bytes, in order to maximize the hardware computation efficiency. \kt{Chen please update these numbers}.
This inspires us to create a \textit{compatibility layer} that can be dynamically allocated and used for any kind of KV caches inside the same LLM.


A naive approach of building such compatibility layer is to partition the GPU memory into pages, where the page size is the greatest common denominator (GCD) for different types of KV caches. We then build memory allocators for different types of attention layers on top of the compatibility layers.
However, this solution significantly slows down the LLM inference engine.
This is because most-performant GPU kernels typically requires the KV cache to be contiguous alongside several tensor dimensions, and the GCD solution may have to partition the tensor along that dimension. As a result, people need to customize GPU kernels for a wide range of possible GCDs, which significantly increasing the GPU kernel engineering overhead and still the performance will not match those most-performant GPU kernels. 

% Also these GPU kernels also significantly inflates the package size \zcsay{can others know what is ``package size''?} of inference engine, slowing down the development and deployment of inference engines.


In contrast, we build such compatibility layer by partitioning the GPU memory into large pages with the page size as the lowest common multiplier (LCM) of different KV cache allocation granularity.
We then build different GPU memory allocators for different types of KV caches, where these memory allocators dynamically adjust the GPU memory pool size by allocating / freeing the large pages, and then perform allocation inside their GPU pool.
Such a solution ensures that the KV cache allocation granularity is always a multiplier of the KV cache allocation granularity of existing inference engines, and thus are compatible with the GPU kernels of existing engines.

We build \sys, the first system that allocates GPU memory for LLM applications, by layering the memory allocator into \textit{compatibility layer} using the LCM of different KV cache allocation granularities, and then build \textit{attention-aware} layer that allocates GPU memory on top of them. \zcsay{compatibility layer vs model layer. a little confusing, better to choose another name}

To make \sys practical, we design the algorithm of \tofill{} to minimizes the internel fragmentation (Section ??) and make sure it is compatible with the prefix caching feature in LLM inference engines (Section ??). \zcsay{the space left for prefix caching is too short. Memory management includes allocation and caching, I think we can discuss caching very fluently in intro.} \kt{Let's discuss and figure out the flow to discuss prefix caching}

\zc{Evaluation shows that \sys can improve the maximum batch size by \tofill{} times and improve the serving throughput by \tofill{} times on average on a set of heterogeneous LLMs.}% \kt{Chen please add placeholders here}
% \zcsay{will fill in the last day}

To summarize, the contributions of this paper are:
\begin{itemize}
    \item A GPU memory allocator that minimizes GPU memory fragmentation for those models with heterogeneous attention layers.
    \item A practical implementation, \sys, that is implemented on top of production-level inference engine vLLM and is compatible to a wide range of inference engine features.
    \item \sys improves the serving engine throughput by ??$\times$ without sacrificing request serving latency.
\end{itemize}

\subsection{Zhuohan's version}
\begin{itemize}
    \item \zc{still need: LLM is popular, LLM memory management is important}
    \item Memory management for LLMs are becoming more complicated than before (when vLLM just came out)
    \begin{itemize}
        \item Models become more complicated:
            \begin{itemize}
                \item Sparse attention layers: sliding window/pyramid kv
                \item Mixed with state-space model: Jamba
                \item Multi-modality: llava and llama
                \item Layer sharing (not sure whether this is challenging for existing memory management scheme) \zcsay{prefer not to discuss  layer sharing in this paper, as it is still fixed size pages}
            \end{itemize}
        \item LLM inference optimizations also bring challenges to the memory manager
        \begin{itemize}
            \item Spec decode (need to manage small model's memory)
            \item Prefix caching (how to free kv cache across different layers?)  \zcsay{Prefix caching is much more important than a sub-sub item in paper flow, needs a fluent way to bring it in, but still keep the two-level allocation as the major contribution that we want the readers to remember}
        \end{itemize}
        \item All of above make managing LLM's runtime memory beyond managing a bunch of fixed size pages, which is the main challenge of this paper.
    \end{itemize}
    \item 
    \kt{We probably need to bring in some related work here}
    \zcsay{Prefer to discuss about the unique properties in LLM that leads to a different design with traditional OS, which is our main insight}
        \item Our major technique: Hierarchical memory allocation to handle \zcsay{I like Kuntai's statements on compatibility layer and re-purposing}
        \begin{itemize}
            \item Specifically, two level: Large page and small page.
                \item Large page for functionality xxx, small pages for functionality yyy.
                \item Large pages takes an LCM of sizes of small pages (please don't highlight this that much in the intro. I think this is pretty straight forward)
    \end{itemize}
    \item Some supporting techniques (I don't fully understand this at the moment and we can discuss more tmrw)
    \begin{itemize}
        \item Request Aware Allocation to Reduce Internal Fragmentation (I don't understand this part fully)
        \item Layer grouping (can be discussed together with layer sharing)
        \item Prefix caching support (need to highlight some techniques here).
    \end{itemize}
    \item \zcsay{I like my previous version on supporting techniques part:}
   \zc{ \item Problems
    \begin{itemize}
        \item Memory allocation: how to avoid internal fragmentation in large page
        \item Accelerators like GPUs needs regular pages (with only one page size) to execute efficiently, but we have multiple page sizes now
        \item Cache replacement policies. 1. better cache replacement policies for single type (e.g., for sliding window-based attention) 2. fair replacement policies for different types
    \end{itemize}
\item Solutions
    \begin{itemize}
        \item Memory allocation: request-aware allocation to avoid internal fragmentation
        \item Execution: represent the allocation result of each layer as single-size pages, with minimal changes to the workers
        \item Cache replace policy: flexible interface to custom last access time of different types of pages, unified LRU for fair replacement
    \end{itemize}
    }
\end{itemize}
% \end{itemize}


% \zcsay{extended from Ion's outline (in memory management google doc):)}
% \begin{itemize}
% \item LLM inference workload are memory-bound.
% \item Challenge: 
% \item{\kt{Kuntai Rewrite start}}
% \item{LLM inference workload are quickly growing, and the LLM inference is in general bounded by memory capacity.}
% \item{sdfasdf}
% \item{To alleviate GPU memory pressure, more and more LLMs choose to substitute memory-consuming self-attention to \textit{\textbf{mixing}} different types of attention mechanisms in the same model to handle long context while controlling the size of KV caches (sliding window + self attention), or to handle different types of modalities (self attention + cross attention).}
% \item{Such trend creates new challenges to the memory allocator, as the \textit{\textbf{tensor shape}} and the \textit{\textbf{memory allocation pattern}} are no longer aligned across layers since different layers may use different attention mechanisms.}
% \item{Existing solutions fall short when handling such mix-attention models.}
% \item{Previous work 1: GPU memory virtualization, where the hardware allows a large KV cache tensor to be stored into non-contiguous small pages, but \zc{large malloc overhead, very bad for small models; cross platform support}}
% \item{Previous work 1: PagedAttention, which assumes the memory allocation patterns and the tensor shapes of KV caches are aligned across layers and manage the KV caches on top of this assumption. Advantage: no memory waste when the LLM models only use one types of attention layers across model. Disadvantage: high amount of memory waste when re-purposing it to those models with different types of attentions.}
% \item{Previous work 2: Fix-ratio allcoation (for each types of attention layers, allocate a fixed-size memory pool for its KV cache). This performs well when the size of different types of KV cache size for different layers has a fixed ratio (e.g. }
% \item{\kt{Kuntai rewrite end}}
% \zc{This intro flow only focus on allocation, but prefix caching is also a large part. Should we position prefix caching as a new challenge of the proposed new allocator?}
% \item Inference workloads are growing (maybe give some data that for many users, inference workloads dominate training workloads; probably even for frontier labs, let alone the others)
% % \kt{The sentence is probably a bit too true to feel like i an argument. A possible alternative: LLM inference systems are serving more and more heterogeneous models.}
% \item Despite the increase in the GPU memory over the past 2 years, many inference workloads are still memory bounded \zc{will highlight capacity bound}
% % \kt{After re-read this, this sentence is not spelling out an issue that directly connects to the end-to-end metrics}
% % \kt{Also I heard that the total capacity of HBM manufacturing is bounded, that's probably the main reason of GPU mem}
% \begin{itemize}
%     \item Longer contexts
%     \item MoE model (lower compute density) (\zcsay{we will cover jamba and hunyuan, though no optimization on MoE layer, we can get speedup from larger batch size})
%     \item Large models, e.g., Llama 3 405B
% \end{itemize}

% \item PagedAttention was introduced to address the memory bottleneck by increasing the efficiency of memory allocation, which led to higher throughput and lower costs.
% However, this is no longer enough. Can cite the 78\% memory waste example of mllama.
% \item Why?: Key assumption of PagedAttention: all tokens have the same KV cache size. No longer hold for new models \kt{This sentence is pointing out the phenomena (different tokens have different KV cache sizes) but does not provide a rationale behind it. An example: The key assumption behind PagedAttention is that the attention layers are \textbf{\textit{ homogeneous}} inside the same model, and thus the KV caches has the same shape across different tokens and different layers. However, as more and more techniques are introduced to reduce the KV cache sizes (e.g. sliding window attention, token dropping), or to incorporate with different modalities (e.g. cross attention), the attention layers are becoming more and more \textbf{\textit{heterogeneous}} even inside the same model, resulting in different KV cache sizes for different tokens and layers.} \sout{Models are becoming more complex}  \zc{updated} (e.g.:
%     \begin{itemize}
%         \item multi-modality, different modality may have different number of tokens (mllama, NVLM, flamingo)
%         \item scalable attention techniques like sliding window attention, token drop, \sout{kv cache sharing}
%         \item serving multiple models together (e.g., speculative decoding, LORAs)
%     \end{itemize}
% \item As a result, they require different page sizes, which is a challenge for most memory allocation system
% \item Opportunity: page size are highly aligned ($m\times 2^n$) \kt{There is no direct logic connection between $m\times 2^n$ and we can have practical benefit}, number of different page size is limited. Which is not held in traditional OS memory management
% \item Main idea: two-level allocation, level0 as the lcm of all page size, and some more details. Highlight this is different from OS memory allocation 
% \item Problems
%     \begin{itemize}
%         \item Memory allocation: how to avoid internal fragmentation in level0 page
%         \item Accelerators like GPUs needs regular pages (with only one page size) to execute efficiently
%         \item Cache replacement policies. 1. better cache replacement policies for single type (e.g., for sliding window-based attention) 2. fair replacement policies for different types
%     \end{itemize}
% \item Solutions
%     \begin{itemize}
%         \item Memory allocation: pages of the same request and nearby tokens usually free together or in nearby time step, so we make best effort to let level1 pages in the same level0 page belongs to same request
%         \item Execution: bias based allocation (see Milestone 1 of google doc), need to summarize the high level idea
%         \item Cache replace policy: flexible interface to custom last access time of different types of pages, two-level LRU for fair replacement
%     \end{itemize}
% \item Evaluation shows that xxxx
% \item Contributions: xxx

% page size is not the key problem
% how allocate, how use(todo refine, shared kv), how drop it
% % and 
% % Solution:
% % multiple page sizes
% % Problem: how do you do it so you can limit fragmentation and don’t hurt performance (i.e., access times). 
% % Solution: 
% % Two-level…

% % Somewhere we need to emphasize this is a new memory organization not used before in OSes.

% \end{itemize}

% \zcsay{
% heterogeneous -> token have different types of memory and shapes. \\
% different shape -> allocation fragmentation \\
% different type -> different hit rule \& fair prefix caching


% problem: all three types of work cannot do allocation. Not list related work on prefix caching
% }

% \zcsay{
% we need to design a new memory allocator. 
% It has new challenge in prefix caching.
% Problem: not our sys cause challenge in prefix caching, but heterogeneous
% }


% 8. Insight: empirically, in order to be hardware-compute-friendly, the KV cache size allocation granularity are pre-determined, limited number of types, and  before runtime, and between different layers simultaneously have a very large GCD (2^10) and a relatively small LCM (<10x GCD). 


% 7. However, all possible types of memory are pre-known and the number is limited, so we can partition the memory that compatible to all types, and further partition it as needed. Specifically, LCM, ..., 

% LCM: not need to change kernel

% LCM good: small size is not bottlenecck, allow small fragementation


% Why previous work is not enough: the size ratio between different attention layer's KV caches can be hugely different between requests, but the allocated KV cache space ratio for different attention layers are the same.



% 6. Our insight: previous work has a static mapping between tensor tokens and KV cache addresses

% 6. Our insight: previous work cannot repurposed the same memory for different tokens with different shapes.

% 6. Our insight: the allocation of previous work are fine-grained on tokens but coarse-grained on model layers -- it allocates KV caches for all layers simultaneously

% 6. Our insight: previous work lacks the ability of allocating different size of memory (not fundamental enough)-> due to xxx  LLM's special property, we can do it by xxx.

% 6. all appoaches somehow introduce a fix size, lacks flexibility for allocate different size memory

% 6. All approaches partition the whole memory space into pre-defined static pieces (fixed-size pages in Paged Attention and vAttention, fixed ratio in fixed size partition), and cannot handle the dynamic scenarios where both the size of each components and the memory size ratio of different types of memory are changing.


% Our insight: previous work 


% Goal: we aim to design a memory allocator in LLM inference engines that can serve heterogeneous models with low memory fragmentation.
% \zcsay{then you need to prove we are compatible with ALL inference engine features}

% \kt{
% Flow 2: we aim to design an in-GPU KV cache caching system for heterogeneous models. Challenge:
% 1. cache tensors with different shapes while maximizing memory efficiency
% 2. eviction
% }

% \zcsay{
\subsection{11/29 Kuntai \& Chen}
\begin{itemize}
\item LLMs are changing the world.
\item LLM inference is growing in importance due to the generality of LLMs (i.e., you don't need to train a new model for each task) and test-time inference/compute.
\item LLM inference is hugely expensive; making it efficient is the key.
\item (Remind people how did we get to vLLM) Token generation is sequential $\rightarrow$ batches to improve parallelism but memory becomes a bottleneck $\rightarrow$ page attention to improve memory utilization and increase batch size.
\item Many things have changed since PagedAttention has been introduced (e.g., multi-modal models, mixed state-space, etc) $\rightarrow$ The result: we need to support multiple types  \zcsay{why it is hard?}

\item Two ways it has changed: (1) different embedding sizes and (2) different data access patterns to reduce computation overhead (e.g., window-based attention). 

\item To address (1) we want to still have equal 

(ion's flow end)
\item New requirement for the memory allocation: how to express the \textit{heterogeneous} allocate / \cred{access} /free patterns of different types, while allowing any types to expand their memory pool using the memory freed by other types.


\item system architecture: two-level memory allocator. Base memory allocator that allocate memory using a page size compatible with all types + customization layer that borrow / return memory from the base memory allocator and executes customized allocation logic in the borrowed memory.

\item Why this is doable: LLMs are heterogeneous, but the heterogeneity inside one single LLM is relatively limited, so it will not create large overhead by designing such base layer.


\item in detail, memory allocation: compatible page size (which is LCM), and different page size for each type; prefix caching: customzed strategy for each type, compatible fair eviction for different types

\item Practical problems
    \begin{itemize}
        \item Memory allocation: how to avoid internal fragmentation in large page
        \item Accelerators like GPUs needs regular pages (with only one page size) to execute efficiently, but we have multiple page sizes now
        \item Allow each type to customize cache management strategy flexibly % Cache replacement policies. ) 2. fair replacement policies for different types
    \end{itemize}
\item Solutions
    \begin{itemize}
        \item Memory allocation: request-aware allocation to avoid internal fragmentation
        \item Execution: represent the allocation result of each layer as single-size pages, with minimal changes to the workers
        \item Cache replace policy: flexible interface to custom last access time of different types of pages %, unified LRU for fair replacement
    \end{itemize}
\end{itemize}

\zc{show new eviction policy as our contribution}

% \kt{
% 7. Two functionalities: 1. which memory need to be allocated (allocation) 2. what should be the type of that allocated memory (instantiation)
% We argue that, we should decouple these two dec
% which memory need to be allocated to what type.
% We argue that we should implement \textit{multiple} memory allocators to allow the allocation / free of different types to decouple with other types, while these multiple memory allocators need 
% }


% 1) which memory should be allocated to which type
% 2) how to use this piece of memory

% how to customize the allocate / \cred{access, need replace} /free patterns of the heterogeneous types, while allowing these customized memory access patterns compatible with each other

% how to customized the usage of memory of hetergeneous type, while allowing these things to exchange memory with each other as needed.

% \item We argue for a \textit{two-layer} desi

% \item Insight: we design a new that can be repurposed 
% \item then, two questions: 1) how to express the unique memory patterns of different component 2) how to fairly and efficiently distributed the overall memory resource to different types

\subsection{12/03 Woosuk}



==> intro_v3.tex <==
\section{Introduction}

% {Ion's Proposed Flow:
% \begin{itemize}
% \item LLMs are changing the world.
% \item LLM inference is growing in importance due to the generality of LLMs (i.e., you don't need to train them for each task) and test-time inference/compute.
% \item LLM inference is hugely expensive; making it efficient is the key.
% \item (Remind people how did we get to vLLM) Token generation is sequential $\rightarrow$ batches to improve parallelism but memory becomes a bottleneck $\rightarrow$ page attention to improve memory utilization and increase batch size.
% \item Many things have changed since PagedAttention has been introduced (e.g., multi-modal models, mixed state-space, etc) $\rightarrow$ The result: we need to support multiple embedding sizes. 
% \item So key challenge is to support multiple embedding sizes and maximize mem utilization. One solution is to have larger page sizes but can lead to internal fragmentation.  
% \item Our solution: two-level memory management based on LCM.
% \item Also heterogeneity brings new (fundamental) challenges to how we do eviction, caching.
% \item ...
% \end{itemize}
% }

% \subsection{Kuntai's version}
% \woosuk{I think the current flow has too many hops. Why don't we start from directly pointing out the difficulty of managing heterogeneous memory states?
% Also, I think we should not focus too much on fragmentation and memory waste, since it does not include prefix caching for heterogeneous layers.}

% Large language models (LLMs) are becoming more and more popular. Billions of people use ChatGPT~\tocite{}, and millions of people use Github Copilot to write code and documentations~\tocite{}.
% To handle huge LLM workload, people find that it is crucial to enlarge LLM inference \textit{batch size}, which allows more requests to be processed within single LLM forwarding pass while only marginally increase the LLM forwarding latency~\tocite{}. \zhuohan{Why talk about batch size here? I feel the concept of batch size comes out of the blue and seems unnecessary here.} \zcsay{we need to point out why avoiding memory waste is important}
% % without  is to perform LLM inference with as large batch size as possible, so that 
% % maximally enlarge the LLM inference batch size, by designing a GPU memory allocator that can fit as many requests into the GPU memory as the GPU memory permits.
% Based on such insight, people develop LLM inference engines (e.g., vLLM~\tocite{} and TGI~\tocite{}) that maximally increase the batch size (by using customized GPU memory allocator to fit as many requests into GPU memory as possible) and thus serve LLM inference requests with much high throughput without inflating the end-to-end latency.

% % \zcsay{We need to highlight batch size is important here, instead of saying "they have good batch size".}
% % \kt{My feeling is that we need to spend a lot of text in intro if we want to explain why large batch size leads to higher throughput (and this text does not really push the logic forward). }
% % Let me try: Due to the xxx property of LLM serving, the throughput of these inference engines highly depends on the number of LLM inference requests that can be batched together, so they design memory allocators to maximally batches as many LLM inference requests as the GPU memory permits}


% Alongside the significant rise of LLM inference workloads, LLM architectures also get increasingly \textit{heterogeneous}, where LLMs use traditional attention layers \textbf{\textit{together with}} other types of attention layer to better customize the model for specific user needs, while maximally preserving the accuracy of the models. 
% For example, \llama 3.2~\cite{dubey2024llama} leverages cross-attention layers for image tokens to handle multi-modality inputs; \gemma~\cite{team2024gemma} leverages sliding window attention layer to better control the KV cache sizes when handling long input context.
% % , or representing all historical information into a very large but fixed size of tensor (e.g. mamba)
% Such heterogeneous attention layers also generate KV caches (the intermediate data of attention layers that need to be cached to generate new tokens) with \textit{different KV cache granularities} (we define the KV cache granularity as the KV cache size for one single token) and \textit{for different sets of tokens}.

% % For example, \llama 3.2 generates KV cache for image tokens and text tokens seperately, where the KV cache granularity for each text token is $4\times$ larger than that of image tokens. 

% As a result, the research question of this paper is: How to design a GPU memory allocator for LLM inference engines that allows maximum batch size for heterogeneous LLM architectures by allocating KV caches with minimum GPU memory fragmentation?

% % There are three types of prior work that handles this challenge, but they all introduces significant memory waste. \zcsay{Related work part is a little long, is it possible to only discuss paged attention here, and put other parts in a seperate discussion section?}

% Existing inference engines tackle this research question by PagedAttention.
% The key innovations of PagedAttention is that it allows partitioning the KV caches generated by LLMs along token dimensions and store each piece of partitioned KV cache into non-adjacent GPU memory addresses, with minimum impact on LLM inference performance.
% % Concretely, it calculates the amount of GPU memory consumed by LLM when handling a fixed amount of tokens (by default 16 in vLLM), and then partitions the GPU memory into pages using such value.
% Such PagedAttention-based inference engines has very low GPU memory fragmentation when handling those models that only uses one type of attention layers.
% However, PagedAttention has significant GPU memory fragmentation when supporting LLMs that use different types of attention layers.
% Concretely \kt{Quantify the amount of memory waste here} %\zcsay{TODO: show the memory waste calculated in sec 3}.

% The key reason behind such GPU memory fragmentation is that PagedAttention's GPU memory allocation strategy is \textit{agnostic} to different types of attention layers, resulting in fixed GPU memory allocation ratio between different attention layer types.
% However, the ratio between the actual GPU memory required by the KV cache of different attention layer types \textit{hugely varies} between different batches.
% \kt{Quantify how much such allocation ratio can vary.}
% As a result, the GPU memory fragmentation can be substantial when the fixed allocation ratio significantly mismatches the actual ratio for the current batch.

% % approaches shares the same limitation: they all partition the whole memory space into pre-defined static pieces (fixed-size pages in Paged Attention and vAttention, fixed ratio in fixed size partition), but the optimal KV cache size partition for different attention layers hugely depends on the context length, and thus vary a lot between different batches.

% % The second type of work is vAttention that allows the LLM applications to allocate large tensors, while the under GPU driver partitions the tensor into small pages (each page is of size 64KB) and performs memory allocation based on such small pages. 
% % This design offloads the memory allocation complexity to GPU drivers, which introduces much higher engineering overhead compared to performing memory allocation inside LLM serving engines, as GPU drivers are much difficult to program, and the effort of changing the driver cannot be reused by other types of GPUs. \zcsay{not true, discussion needed}

% % The third type of work is creating a fix-size memory pool for different types of KV caches, and then perform memory allocation inside each pool. 
% % As a result, the GPU memory allocation ratio between different types of attention layers are fixed, and result in high memory waste when serving models with different types of attentions.

% We argue that: instead of fixing the ratio of GPU memory size between different types of attention layers, the memory allocator needs to be able to \textbf{\textit{dynamically}} adjust such ratio to match the actual GPU memory requirement ratio of the current LLM inference batch.

% Such dynamic memory allocation is in general difficult and motivates decades of research~\tocite{}.
% However, in LLM applications, such problem is much simpler to tackle: though different LLMs have highly heterogeneous attention layers, empirically we observe that the heterogeneity inside the same LLM is much more \textbf{\textit{limited}}. 
% Concretely, a typical LLM uses at most 3 different types of attention layers, and the size of those KV caches are typically a multiplier of $2^{10}$ bytes, in order to maximize the hardware computation efficiency. \kt{Chen please update these numbers}.
% This inspires us to create a \textit{compatibility layer} that can be dynamically allocated and used for any kind of KV caches inside the same LLM.


% A naive approach of building such compatibility layer is to partition the GPU memory into pages, where the page size is the greatest common denominator (GCD) for different types of KV caches. We then build memory allocators for different types of attention layers on top of the compatibility layers.
% However, this solution significantly slows down the LLM inference engine.
% This is because most-performant GPU kernels typically requires the KV cache to be contiguous alongside several tensor dimensions, and the GCD solution may have to partition the tensor along that dimension. As a result, people need to customize GPU kernels for a wide range of possible GCDs, which significantly increasing the GPU kernel engineering overhead and still the performance will not match those most-performant GPU kernels. 

% % Also these GPU kernels also significantly inflates the package size \zcsay{can others know what is ``package size''?} of inference engine, slowing down the development and deployment of inference engines.


% In contrast, we build such compatibility layer by partitioning the GPU memory into large pages with the page size as the lowest common multiplier (LCM) of different KV cache allocation granularity.
% We then build different GPU memory allocators for different types of KV caches, where these memory allocators dynamically adjust the GPU memory pool size by allocating / freeing the large pages, and then perform allocation inside their GPU pool.
% Such a solution ensures that the KV cache allocation granularity is always a multiplier of the KV cache allocation granularity of existing inference engines, and thus are compatible with the GPU kernels of existing engines.

% We build \sys, the first system that allocates GPU memory for LLM applications, by layering the memory allocator into \textit{compatibility layer} using the LCM of different KV cache allocation granularities, and then build \textit{attention-aware} layer that allocates GPU memory on top of them. \zcsay{compatibility layer vs model layer. a little confusing, better to choose another name}

% To make \sys practical, we design the algorithm of \tofill{} to minimizes the internel fragmentation (Section ??) and make sure it is compatible with the prefix caching feature in LLM inference engines (Section ??). \zcsay{the space left for prefix caching is too short. Memory management includes allocation and caching, I think we can discuss caching very fluently in intro.} \kt{Let's discuss and figure out the flow to discuss prefix caching}

% \zc{Evaluation shows that \sys can improve the maximum batch size by \tofill{} times and improve the serving throughput by \tofill{} times on average on a set of heterogeneous LLMs.}% \kt{Chen please add placeholders here}
% % \zcsay{will fill in the last day}

% To summarize, the contributions of this paper are:
% \begin{itemize}
%     \item A GPU memory allocator that minimizes GPU memory fragmentation for those models with heterogeneous attention layers.
%     \item A practical implementation, \sys, that is implemented on top of production-level inference engine vLLM and is compatible to a wide range of inference engine features.
%     \item \sys improves the serving engine throughput by ??$\times$ without sacrificing request serving latency.
% \end{itemize}

% \subsection{Zhuohan's version}
% \begin{itemize}
%     \item \zc{still need: LLM is popular, LLM memory management is important}
%     \item Memory management for LLMs are becoming more complicated than before (when vLLM just came out)
%     \begin{itemize}
%         \item Models become more complicated:
%             \begin{itemize}
%                 \item Sparse attention layers: sliding window/pyramid kv
%                 \item Mixed with state-space model: Jamba
%                 \item Multi-modality: llava and llama
%                 \item Layer sharing (not sure whether this is challenging for existing memory management scheme) \zcsay{prefer not to discuss  layer sharing in this paper, as it is still fixed size pages}
%             \end{itemize}
%         \item LLM inference optimizations also bring challenges to the memory manager
%         \begin{itemize}
%             \item Spec decode (need to manage small model's memory)
%             \item Prefix caching (how to free kv cache across different layers?)  \zcsay{Prefix caching is much more important than a sub-sub item in paper flow, needs a fluent way to bring it in, but still keep the two-level allocation as the major contribution that we want the readers to remember}
%         \end{itemize}
%         \item All of above make managing LLM's runtime memory beyond managing a bunch of fixed size pages, which is the main challenge of this paper.
%     \end{itemize}
%     \item 
%     \kt{We probably need to bring in some related work here}
%     \zcsay{Prefer to discuss about the unique properties in LLM that leads to a different design with traditional OS, which is our main insight}
%         \item Our major technique: Hierarchical memory allocation to handle \zcsay{I like Kuntai's statements on compatibility layer and re-purposing}
%         \begin{itemize}
%             \item Specifically, two level: Large page and small page.
%                 \item Large page for functionality xxx, small pages for functionality yyy.
%                 \item Large pages takes an LCM of sizes of small pages (please don't highlight this that much in the intro. I think this is pretty straight forward)
%     \end{itemize}
%     \item Some supporting techniques (I don't fully understand this at the moment and we can discuss more tmrw)
%     \begin{itemize}
%         \item Request Aware Allocation to Reduce Internal Fragmentation (I don't understand this part fully)
%         \item Layer grouping (can be discussed together with layer sharing)
%         \item Prefix caching support (need to highlight some techniques here).
%     \end{itemize}
%     \item \zcsay{I like my previous version on supporting techniques part:}
%    \zc{ \item Problems
%     \begin{itemize}
%         \item Memory allocation: how to avoid internal fragmentation in large page
%         \item Accelerators like GPUs needs regular pages (with only one page size) to execute efficiently, but we have multiple page sizes now
%         \item Cache replacement policies. 1. better cache replacement policies for single type (e.g., for sliding window-based attention) 2. fair replacement policies for different types
%     \end{itemize}
% \item Solutions
%     \begin{itemize}
%         \item Memory allocation: request-aware allocation to avoid internal fragmentation
%         \item Execution: represent the allocation result of each layer as single-size pages, with minimal changes to the workers
%         \item Cache replace policy: flexible interface to custom last access time of different types of pages, unified LRU for fair replacement
%     \end{itemize}
%     }
% \end{itemize}
% % \end{itemize}


% \zcsay{extended from Ion's outline (in memory management google doc):)}
% \begin{itemize}
% \item LLM inference workload are memory-bound.
% \item Challenge: 
% \item{\kt{Kuntai Rewrite start}}
% \item{LLM inference workload are quickly growing, and the LLM inference is in general bounded by memory capacity.}
% \item{sdfasdf}
% \item{To alleviate GPU memory pressure, more and more LLMs choose to substitute memory-consuming self-attention to \textit{\textbf{mixing}} different types of attention mechanisms in the same model to handle long context while controlling the size of KV caches (sliding window + self attention), or to handle different types of modalities (self attention + cross attention).}
% \item{Such trend creates new challenges to the memory allocator, as the \textit{\textbf{tensor shape}} and the \textit{\textbf{memory allocation pattern}} are no longer aligned across layers since different layers may use different attention mechanisms.}
% \item{Existing solutions fall short when handling such mix-attention models.}
% \item{Previous work 1: GPU memory virtualization, where the hardware allows a large KV cache tensor to be stored into non-contiguous small pages, but \zc{large malloc overhead, very bad for small models; cross platform support}}
% \item{Previous work 1: PagedAttention, which assumes the memory allocation patterns and the tensor shapes of KV caches are aligned across layers and manage the KV caches on top of this assumption. Advantage: no memory waste when the LLM models only use one types of attention layers across model. Disadvantage: high amount of memory waste when re-purposing it to those models with different types of attentions.}
% \item{Previous work 2: Fix-ratio allcoation (for each types of attention layers, allocate a fixed-size memory pool for its KV cache). This performs well when the size of different types of KV cache size for different layers has a fixed ratio (e.g. }
% \item{\kt{Kuntai rewrite end}}
% \zc{This intro flow only focus on allocation, but prefix caching is also a large part. Should we position prefix caching as a new challenge of the proposed new allocator?}
% \item Inference workloads are growing (maybe give some data that for many users, inference workloads dominate training workloads; probably even for frontier labs, let alone the others)
% % \kt{The sentence is probably a bit too true to feel like i an argument. A possible alternative: LLM inference systems are serving more and more heterogeneous models.}
% \item Despite the increase in the GPU memory over the past 2 years, many inference workloads are still memory bounded \zc{will highlight capacity bound}
% % \kt{After re-read this, this sentence is not spelling out an issue that directly connects to the end-to-end metrics}
% % \kt{Also I heard that the total capacity of HBM manufacturing is bounded, that's probably the main reason of GPU mem}
% \begin{itemize}
%     \item Longer contexts
%     \item MoE model (lower compute density) (\zcsay{we will cover jamba and hunyuan, though no optimization on MoE layer, we can get speedup from larger batch size})
%     \item Large models, e.g., Llama 3 405B
% \end{itemize}

% \item PagedAttention was introduced to address the memory bottleneck by increasing the efficiency of memory allocation, which led to higher throughput and lower costs.
% However, this is no longer enough. Can cite the 78\% memory waste example of mllama.
% \item Why?: Key assumption of PagedAttention: all tokens have the same KV cache size. No longer hold for new models \kt{This sentence is pointing out the phenomena (different tokens have different KV cache sizes) but does not provide a rationale behind it. An example: The key assumption behind PagedAttention is that the attention layers are \textbf{\textit{ homogeneous}} inside the same model, and thus the KV caches has the same shape across different tokens and different layers. However, as more and more techniques are introduced to reduce the KV cache sizes (e.g. sliding window attention, token dropping), or to incorporate with different modalities (e.g. cross attention), the attention layers are becoming more and more \textbf{\textit{heterogeneous}} even inside the same model, resulting in different KV cache sizes for different tokens and layers.} \sout{Models are becoming more complex}  \zc{updated} (e.g.:
%     \begin{itemize}
%         \item multi-modality, different modality may have different number of tokens (mllama, NVLM, flamingo)
%         \item scalable attention techniques like sliding window attention, token drop, \sout{kv cache sharing}
%         \item serving multiple models together (e.g., speculative decoding, LORAs)
%     \end{itemize}
% \item As a result, they require different page sizes, which is a challenge for most memory allocation system
% \item Opportunity: page size are highly aligned ($m\times 2^n$) \kt{There is no direct logic connection between $m\times 2^n$ and we can have practical benefit}, number of different page size is limited. Which is not held in traditional OS memory management
% \item Main idea: two-level allocation, level0 as the lcm of all page size, and some more details. Highlight this is different from OS memory allocation 
% \item Problems
%     \begin{itemize}
%         \item Memory allocation: how to avoid internal fragmentation in level0 page
%         \item Accelerators like GPUs needs regular pages (with only one page size) to execute efficiently
%         \item Cache replacement policies. 1. better cache replacement policies for single type (e.g., for sliding window-based attention) 2. fair replacement policies for different types
%     \end{itemize}
% \item Solutions
%     \begin{itemize}
%         \item Memory allocation: pages of the same request and nearby tokens usually free together or in nearby time step, so we make best effort to let level1 pages in the same level0 page belongs to same request
%         \item Execution: bias based allocation (see Milestone 1 of google doc), need to summarize the high level idea
%         \item Cache replace policy: flexible interface to custom last access time of different types of pages, two-level LRU for fair replacement
%     \end{itemize}
% \item Evaluation shows that xxxx
% \item Contributions: xxx

% page size is not the key problem
% how allocate, how use(todo refine, shared kv), how drop it
% % and 
% % Solution:
% % multiple page sizes
% % Problem: how do you do it so you can limit fragmentation and don’t hurt performance (i.e., access times). 
% % Solution: 
% % Two-level…

% % Somewhere we need to emphasize this is a new memory organization not used before in OSes.

% \end{itemize}

% \zcsay{
% heterogeneous -> token have different types of memory and shapes. \\
% different shape -> allocation fragmentation \\
% different type -> different hit rule \& fair prefix caching


% problem: all three types of work cannot do allocation. Not list related work on prefix caching
% }

% \zcsay{
% we need to design a new memory allocator. 
% It has new challenge in prefix caching.
% Problem: not our sys cause challenge in prefix caching, but heterogeneous
% }


% 8. Insight: empirically, in order to be hardware-compute-friendly, the KV cache size allocation granularity are pre-determined, limited number of types, and  before runtime, and between different layers simultaneously have a very large GCD (2^10) and a relatively small LCM (<10x GCD). 


% 7. However, all possible types of memory are pre-known and the number is limited, so we can partition the memory that compatible to all types, and further partition it as needed. Specifically, LCM, ..., 

% LCM: not need to change kernel

% LCM good: small size is not bottlenecck, allow small fragementation


% Why previous work is not enough: the size ratio between different attention layer's KV caches can be hugely different between requests, but the allocated KV cache space ratio for different attention layers are the same.



% 6. Our insight: previous work has a static mapping between tensor tokens and KV cache addresses

% 6. Our insight: previous work cannot repurposed the same memory for different tokens with different shapes.

% 6. Our insight: the allocation of previous work are fine-grained on tokens but coarse-grained on model layers -- it allocates KV caches for all layers simultaneously

% 6. Our insight: previous work lacks the ability of allocating different size of memory (not fundamental enough)-> due to xxx  LLM's special property, we can do it by xxx.

% 6. all appoaches somehow introduce a fix size, lacks flexibility for allocate different size memory

% 6. All approaches partition the whole memory space into pre-defined static pieces (fixed-size pages in Paged Attention and vAttention, fixed ratio in fixed size partition), and cannot handle the dynamic scenarios where both the size of each components and the memory size ratio of different types of memory are changing.


% Our insight: previous work 


% Goal: we aim to design a memory allocator in LLM inference engines that can serve heterogeneous models with low memory fragmentation.
% \zcsay{then you need to prove we are compatible with ALL inference engine features}

% \kt{
% Flow 2: we aim to design an in-GPU KV cache caching system for heterogeneous models. Challenge:
% 1. cache tensors with different shapes while maximizing memory efficiency
% 2. eviction
% }

% \zcsay{
% \subsection{11/29 Kuntai \& Chen}
% \begin{itemize}
Large language models (LLMs) are becoming popular. Billions of people use ChatGPT~\tocite{}, and millions of people use Github Copilot to write code and documentations~\tocite{}. As a result, the LLM inference workload is rapidly growing. 

However, LLM inference requests are expensive to serve. One single H100 GPU costs \$\tofill{}, and it can only fit a medium-size (e.g. Llama 8B) LLM into memory and serve \tofill{} requests per second, if the requests are processed one-by-one.
The key reason behind such inefficiency is that a single LLM request cannot fully saturate the GPU's parallel computing capability. This is because LLMs are auto-regressive models that have to generate tokens one-by-one and thus cannot generate multiple tokens in parallel. \zcsay{prefer to simplify this paragraph, just mention it is expensive in one sentence} \kt{I am already reducing the points compared to Ion's outline. Shall we keep simplifying it?}

As a result, to accelerate LLM inference, previous work proposes that LLM inference needs to be massively batched in order to saturate GPU's parallel computing capability. 
Such massive batching challenges the GPU memory management system design, as the KV cache, the intermediate tensors generated by LLM's attention module that can be large, of all requests in the batch needs to be stored on GPU in order to perform batched inference.
Further, there is another key optimization, \textit{prefix caching}, that requires careful design of GPU memory management system.
Prefix caching is a technique that requires the GPU memory management system to keep the KV cache for one request in GPU, so that it can be reused by another request, if those two requests share the same prefix.
Thus, the GPU memory management system also needs to 

PagedAttention provides a practical solution for those LLMs that only use self-attention attention mechanism, which is a valid assumption for early-stage LLMs.

However, LLM models becoming more and more heterogeneous.
Concretely, people will \textbf{\textit{mix}} traditional attention layers \textbf{\textit{together with}} other types of attention layer to customize the model for specific user needs. 
For example, \llama 3.2~\cite{dubey2024llama} leverages cross-attention layers for image tokens to handle multi-modality inputs; \gemma~\cite{team2024gemma} leverages sliding window attention layers to better control the KV cache sizes when handling long input context.
As a result, the KV caches inside one single model is also becoming heterogeneous and will have different sizes and life cycles.
Concretely, \tofill{} \kt{Chen can you fill in an example here} \zcsay{I suggest draw hymba and explain it. also need jamba in the paragraph, as mllama and gemma has same hidden size per layer, which is not complex enough} \zcsay{seems that different life-cycle is only in prefix caching part. memory allocator does not make special design for this} \kt{I agree that memory allocator typically has nothing to do with caching. But we need a new word similar to memory allocator to illustrate the thing \sys is building, what should it be other than memory allocator?} \zcsay{I'm using memory management system / memory manager} \cred{to discuss: play with hamba}

As a result, our goal is to design a GPU memory allocator to maximally utilize GPU memory for those LLMs that uses different attention layers and generates different sizes of KV caches with different KV cache life cycles? \zcsay{need to explain different kv cache sizes and different lifecycle before this paragraph} \kt{The last paragraph did that} \zcsay{I don't think so. let's discuss}

The general form of this question (i.e. memory allocation for different sizes of objects with different life cycles) is extremely challenging and motivates decades of research~\tocite{}.
In LLM applications, however, such problem is much easier to tackle: even though the LLMs can be hugely heterogeneous, the heterogeneity inside one single LLM is relatively limited.
Concretely, we make the following empirical observations:
\begin{itemize}
    \item The number of different types of KV caches is relatively limited: at most five different types KV caches need to be stored in GPU when serving a LLM. \kt{This argument does not directly motivate the compatibility itself, instead it argues that if we do compatible layer, the overhead is small. So it is probably not a good argument for here.} \cred{VOTE}
    \item KV cache sizes inside the same LLM are typically a multiplier of \cred{$2^{10}$} bytes, \cred{as this ensures that the computation on top of KV caches can be easily parallelized by the CUDA kernel and among multiple GPUs.} 
    As a result, it is possible to find a \textit{compatible size}, where not only different types of KV caches can perform memory allocation on top of such compatible size with little internal memory fragmentation, and it allows the GPU memory freed by one types of KV caches can be reused by another.
    % \zc{KV cache sizes inside the same LLM are typically a multiplier of \cred{$2^{10}$} bytes due to the parallelization requirement of GPU architecture. The highly-aligned KV cache size makes compatible page size possible}
   \item Life-cycle-wise, though different types of KV cache can have hugely-different life cycles, they only rely on two operators to controls the life cycles: \textit{extend} the original KV cache pool size by one token, or \textit{drop} the KV caches for one of the previous tokens. As a result, we can implement these two APIs first, and then implement customized logic for different types of KV caches by calling these two APIs. \kt{Chen can you make sure if these are the two APIs we use? If not, let's discuss if there is a set of API we can introduce without diving into too much details of prefix caching} \zcsay{see \Cref{fig:interface}}
   \cred{Current best answer: different types of KV caches all need to customize their prefix caching policy based on the workload to achieve best performance.}
   \cred{A weaker argument: some KV caches no longer need to be stored in GPU if its dependent KV caches are evicted }
\end{itemize}

\zcsay{some pages need to hit together, challenging to cache system}
\zcsay{the importance of tokens of current request: the longer the important. the importance for future requests: this property not hold (e.g., system prompt, long context qa)}

These observations inspire us to build two-level GPU memory allocator, where the base memory allocator allocates memory using a page size compatible with different KV cache sizes, and the customizable allocators borrow and return memory from the base memory allocator, and executes customized allocation logic to manage the life cycle of different KV caches. 
Based on such insight, we propose \sys, the first GPU memory allocator that maximizes GPU memory utilization for heterogeneous LLMs that uses traditional self-attention together with other types of attentions.
\zcsay{the solution is a little abstract, need to make it more detail}
\kt{I don't know the techniques much so Chen can you write it?}

The practical challenge of \sys is: how to support the widely-used prefix caching optimization, so that the KV caches computed by one request can be reused by another request with the same prefix?
To handle this challenge, we engineer the allocation, caching and eviction logic for a wide range of attention layers, so that it is compatible with the prefix caching feature of existing LLM inference engines, while making sure that the prefix cache eviction is fair for different types of KV caches. \zcsay{does the discussions before this paragraph include prefix caching? I think including prefix caching like this is quite strange}

We evaluate on \sys on \tofill{} LLMs, \tofill{} datasets and \tofill{} GPUs. Our evaluation shows that, compared to state-of-the-art LLM serving engine vLLM, \sys achieves \tofill{}x higher throughput without hurting the end-to-end latency, by maximally batching LLM inference requests with little memory waste. Also, \sys is significant under different GPUs. \sys is also compatible with a wide range of features in LLM serving engines.

To summarize, the contribution of this paper is as follows:
\begin{packeditemize}
    \item A GPU memory allocator that improves throughput for those LLMs with differet KV cache sizes and life cycles, by maximally batch requests with minimum GPU memory waste. \zcsay{add also clever prefix caching?}
    \item A practical implementation, \sys, that is implemented on top of production-level inference engine vLLM and is compatible to a wide range of inference engine features.
    \item \sys improves the serving engine throughput by \tofill{}$\times$ without sacrificing request serving latency.
\end{packeditemize}

% \item Practical problems
%     \begin{itemize}
%         \item Memory allocation: how to avoid internal fragmentation in large page
%         \item Accelerators like GPUs needs regular pages (with only one page size) to execute efficiently, but we have multiple page sizes now
%         \item Allow each type to customize cache management strategy flexibly % Cache replacement policies. ) 2. fair replacement policies for different types
%     \end{itemize}
% \item Solutions
%     \begin{itemize}
%         \item Memory allocation: request-aware allocation to avoid internal fragmentation
%         \item Execution: represent the allocation result of each layer as single-size pages, with minimal changes to the workers
%         \item Cache replace policy: flexible interface to custom last access time of different types of pages %, unified LRU for fair replacement
%     \end{itemize}
% \end{itemize}

% \zc{show new eviction policy as our contribution}

% \kt{
% 7. Two functionalities: 1. which memory need to be allocated (allocation) 2. what should be the type of that allocated memory (instantiation)
% We argue that, we should decouple these two dec
% which memory need to be allocated to what type.
% We argue that we should implement \textit{multiple} memory allocators to allow the allocation / free of different types to decouple with other types, while these multiple memory allocators need 
% }


% 1) which memory should be allocated to which type
% 2) how to use this piece of memory

% how to customize the allocate / \cred{access, need replace} /free patterns of the heterogeneous types, while allowing these customized memory access patterns compatible with each other

% how to customized the usage of memory of hetergeneous type, while allowing these things to exchange memory with each other as needed.

% \item We argue for a \textit{two-layer} desi

% \item Insight: we design a new that can be repurposed 
% \item then, two questions: 1) how to express the unique memory patterns of different component 2) how to fairly and efficiently distributed the overall memory resource to different types

\subsection{12/03 Woosuk}



==> intro_v4.tex <==
\section{Introduction}

% {Ion's Proposed Flow:
% \begin{itemize}
% \item LLMs are changing the world.
% \item LLM inference is growing in importance due to the generality of LLMs (i.e., you don't need to train them for each task) and test-time inference/compute.
% \item LLM inference is hugely expensive; making it efficient is the key.
% \item (Remind people how did we get to vLLM) Token generation is sequential $\rightarrow$ batches to improve parallelism but memory becomes a bottleneck $\rightarrow$ page attention to improve memory utilization and increase batch size.
% \item Many things have changed since PagedAttention has been introduced (e.g., multi-modal models, mixed state-space, etc) $\rightarrow$ The result: we need to support multiple embedding sizes. 
% \item So key challenge is to support multiple embedding sizes and maximize mem utilization. One solution is to have larger page sizes but can lead to internal fragmentation.  
% \item Our solution: two-level memory management based on LCM.
% \item Also heterogeneity brings new (fundamental) challenges to how we do eviction, caching.
% \item ...
% \end{itemize}
% }

% \subsection{Kuntai's version}
% \woosuk{I think the current flow has too many hops. Why don't we start from directly pointing out the difficulty of managing heterogeneous memory states?
% Also, I think we should not focus too much on fragmentation and memory waste, since it does not include prefix caching for heterogeneous layers.}

% Large language models (LLMs) are becoming more and more popular. Billions of people use ChatGPT~\tocite{}, and millions of people use Github Copilot to write code and documentations~\tocite{}.
% To handle huge LLM workload, people find that it is crucial to enlarge LLM inference \textit{batch size}, which allows more requests to be processed within single LLM forwarding pass while only marginally increase the LLM forwarding latency~\tocite{}. \zhuohan{Why talk about batch size here? I feel the concept of batch size comes out of the blue and seems unnecessary here.} \zcsay{we need to point out why avoiding memory waste is important}
% % without  is to perform LLM inference with as large batch size as possible, so that 
% % maximally enlarge the LLM inference batch size, by designing a GPU memory allocator that can fit as many requests into the GPU memory as the GPU memory permits.
% Based on such insight, people develop LLM inference engines (e.g., vLLM~\tocite{} and TGI~\tocite{}) that maximally increase the batch size (by using customized GPU memory allocator to fit as many requests into GPU memory as possible) and thus serve LLM inference requests with much high throughput without inflating the end-to-end latency.

% % \zcsay{We need to highlight batch size is important here, instead of saying "they have good batch size".}
% % \kt{My feeling is that we need to spend a lot of text in intro if we want to explain why large batch size leads to higher throughput (and this text does not really push the logic forward). }
% % Let me try: Due to the xxx property of LLM serving, the throughput of these inference engines highly depends on the number of LLM inference requests that can be batched together, so they design memory allocators to maximally batches as many LLM inference requests as the GPU memory permits}


% Alongside the significant rise of LLM inference workloads, LLM architectures also get increasingly \textit{heterogeneous}, where LLMs use traditional attention layers \textbf{\textit{together with}} other types of attention layer to better customize the model for specific user needs, while maximally preserving the accuracy of the models. 
% For example, \llama 3.2~\cite{dubey2024llama} leverages cross-attention layers for image tokens to handle multi-modality inputs; \gemma~\cite{team2024gemma} leverages sliding window attention layer to better control the KV cache sizes when handling long input context.
% % , or representing all historical information into a very large but fixed size of tensor (e.g. mamba)
% Such heterogeneous attention layers also generate KV caches (the intermediate data of attention layers that need to be cached to generate new tokens) with \textit{different KV cache granularities} (we define the KV cache granularity as the KV cache size for one single token) and \textit{for different sets of tokens}.

% % For example, \llama 3.2 generates KV cache for image tokens and text tokens seperately, where the KV cache granularity for each text token is $4\times$ larger than that of image tokens. 

% As a result, the research question of this paper is: How to design a GPU memory allocator for LLM inference engines that allows maximum batch size for heterogeneous LLM architectures by allocating KV caches with minimum GPU memory fragmentation?

% % There are three types of prior work that handles this challenge, but they all introduces significant memory waste. \zcsay{Related work part is a little long, is it possible to only discuss paged attention here, and put other parts in a seperate discussion section?}

% Existing inference engines tackle this research question by PagedAttention.
% The key innovations of PagedAttention is that it allows partitioning the KV caches generated by LLMs along token dimensions and store each piece of partitioned KV cache into non-adjacent GPU memory addresses, with minimum impact on LLM inference performance.
% % Concretely, it calculates the amount of GPU memory consumed by LLM when handling a fixed amount of tokens (by default 16 in vLLM), and then partitions the GPU memory into pages using such value.
% Such PagedAttention-based inference engines has very low GPU memory fragmentation when handling those models that only uses one type of attention layers.
% However, PagedAttention has significant GPU memory fragmentation when supporting LLMs that use different types of attention layers.
% Concretely \kt{Quantify the amount of memory waste here} %\zcsay{TODO: show the memory waste calculated in sec 3}.

% The key reason behind such GPU memory fragmentation is that PagedAttention's GPU memory allocation strategy is \textit{agnostic} to different types of attention layers, resulting in fixed GPU memory allocation ratio between different attention layer types.
% However, the ratio between the actual GPU memory required by the KV cache of different attention layer types \textit{hugely varies} between different batches.
% \kt{Quantify how much such allocation ratio can vary.}
% As a result, the GPU memory fragmentation can be substantial when the fixed allocation ratio significantly mismatches the actual ratio for the current batch.

% % approaches shares the same limitation: they all partition the whole memory space into pre-defined static pieces (fixed-size pages in Paged Attention and vAttention, fixed ratio in fixed size partition), but the optimal KV cache size partition for different attention layers hugely depends on the context length, and thus vary a lot between different batches.

% % The second type of work is vAttention that allows the LLM applications to allocate large tensors, while the under GPU driver partitions the tensor into small pages (each page is of size 64KB) and performs memory allocation based on such small pages. 
% % This design offloads the memory allocation complexity to GPU drivers, which introduces much higher engineering overhead compared to performing memory allocation inside LLM serving engines, as GPU drivers are much difficult to program, and the effort of changing the driver cannot be reused by other types of GPUs. \zcsay{not true, discussion needed}

% % The third type of work is creating a fix-size memory pool for different types of KV caches, and then perform memory allocation inside each pool. 
% % As a result, the GPU memory allocation ratio between different types of attention layers are fixed, and result in high memory waste when serving models with different types of attentions.

% We argue that: instead of fixing the ratio of GPU memory size between different types of attention layers, the memory allocator needs to be able to \textbf{\textit{dynamically}} adjust such ratio to match the actual GPU memory requirement ratio of the current LLM inference batch.

% Such dynamic memory allocation is in general difficult and motivates decades of research~\tocite{}.
% However, in LLM applications, such problem is much simpler to tackle: though different LLMs have highly heterogeneous attention layers, empirically we observe that the heterogeneity inside the same LLM is much more \textbf{\textit{limited}}. 
% Concretely, a typical LLM uses at most 3 different types of attention layers, and the size of those KV caches are typically a multiplier of $2^{10}$ bytes, in order to maximize the hardware computation efficiency. \kt{Chen please update these numbers}.
% This inspires us to create a \textit{compatibility layer} that can be dynamically allocated and used for any kind of KV caches inside the same LLM.


% A naive approach of building such compatibility layer is to partition the GPU memory into pages, where the page size is the greatest common denominator (GCD) for different types of KV caches. We then build memory allocators for different types of attention layers on top of the compatibility layers.
% However, this solution significantly slows down the LLM inference engine.
% This is because most-performant GPU kernels typically requires the KV cache to be contiguous alongside several tensor dimensions, and the GCD solution may have to partition the tensor along that dimension. As a result, people need to customize GPU kernels for a wide range of possible GCDs, which significantly increasing the GPU kernel engineering overhead and still the performance will not match those most-performant GPU kernels. 

% % Also these GPU kernels also significantly inflates the package size \zcsay{can others know what is ``package size''?} of inference engine, slowing down the development and deployment of inference engines.


% In contrast, we build such compatibility layer by partitioning the GPU memory into large pages with the page size as the lowest common multiplier (LCM) of different KV cache allocation granularity.
% We then build different GPU memory allocators for different types of KV caches, where these memory allocators dynamically adjust the GPU memory pool size by allocating / freeing the large pages, and then perform allocation inside their GPU pool.
% Such a solution ensures that the KV cache allocation granularity is always a multiplier of the KV cache allocation granularity of existing inference engines, and thus are compatible with the GPU kernels of existing engines.

% We build \sys, the first system that allocates GPU memory for LLM applications, by layering the memory allocator into \textit{compatibility layer} using the LCM of different KV cache allocation granularities, and then build \textit{attention-aware} layer that allocates GPU memory on top of them. \zcsay{compatibility layer vs model layer. a little confusing, better to choose another name}

% To make \sys practical, we design the algorithm of \tofill{} to minimizes the internel fragmentation (Section ??) and make sure it is compatible with the prefix caching feature in LLM inference engines (Section ??). \zcsay{the space left for prefix caching is too short. Memory management includes allocation and caching, I think we can discuss caching very fluently in intro.} \kt{Let's discuss and figure out the flow to discuss prefix caching}

% \zc{Evaluation shows that \sys can improve the maximum batch size by \tofill{} times and improve the serving throughput by \tofill{} times on average on a set of heterogeneous LLMs.}% \kt{Chen please add placeholders here}
% % \zcsay{will fill in the last day}

% To summarize, the contributions of this paper are:
% \begin{itemize}
%     \item A GPU memory allocator that minimizes GPU memory fragmentation for those models with heterogeneous attention layers.
%     \item A practical implementation, \sys, that is implemented on top of production-level inference engine vLLM and is compatible to a wide range of inference engine features.
%     \item \sys improves the serving engine throughput by ??$\times$ without sacrificing request serving latency.
% \end{itemize}

% \subsection{Zhuohan's version}
% \begin{itemize}
%     \item \zc{still need: LLM is popular, LLM memory management is important}
%     \item Memory management for LLMs are becoming more complicated than before (when vLLM just came out)
%     \begin{itemize}
%         \item Models become more complicated:
%             \begin{itemize}
%                 \item Sparse attention layers: sliding window/pyramid kv
%                 \item Mixed with state-space model: Jamba
%                 \item Multi-modality: llava and llama
%                 \item Layer sharing (not sure whether this is challenging for existing memory management scheme) \zcsay{prefer not to discuss  layer sharing in this paper, as it is still fixed size pages}
%             \end{itemize}
%         \item LLM inference optimizations also bring challenges to the memory manager
%         \begin{itemize}
%             \item Spec decode (need to manage small model's memory)
%             \item Prefix caching (how to free kv cache across different layers?)  \zcsay{Prefix caching is much more important than a sub-sub item in paper flow, needs a fluent way to bring it in, but still keep the two-level allocation as the major contribution that we want the readers to remember}
%         \end{itemize}
%         \item All of above make managing LLM's runtime memory beyond managing a bunch of fixed size pages, which is the main challenge of this paper.
%     \end{itemize}
%     \item 
%     \kt{We probably need to bring in some related work here}
%     \zcsay{Prefer to discuss about the unique properties in LLM that leads to a different design with traditional OS, which is our main insight}
%         \item Our major technique: Hierarchical memory allocation to handle \zcsay{I like Kuntai's statements on compatibility layer and re-purposing}
%         \begin{itemize}
%             \item Specifically, two level: Large page and small page.
%                 \item Large page for functionality xxx, small pages for functionality yyy.
%                 \item Large pages takes an LCM of sizes of small pages (please don't highlight this that much in the intro. I think this is pretty straight forward)
%     \end{itemize}
%     \item Some supporting techniques (I don't fully understand this at the moment and we can discuss more tmrw)
%     \begin{itemize}
%         \item Request Aware Allocation to Reduce Internal Fragmentation (I don't understand this part fully)
%         \item Layer grouping (can be discussed together with layer sharing)
%         \item Prefix caching support (need to highlight some techniques here).
%     \end{itemize}
%     \item \zcsay{I like my previous version on supporting techniques part:}
%    \zc{ \item Problems
%     \begin{itemize}
%         \item Memory allocation: how to avoid internal fragmentation in large page
%         \item Accelerators like GPUs needs regular pages (with only one page size) to execute efficiently, but we have multiple page sizes now
%         \item Cache replacement policies. 1. better cache replacement policies for single type (e.g., for sliding window-based attention) 2. fair replacement policies for different types
%     \end{itemize}
% \item Solutions
%     \begin{itemize}
%         \item Memory allocation: request-aware allocation to avoid internal fragmentation
%         \item Execution: represent the allocation result of each layer as single-size pages, with minimal changes to the workers
%         \item Cache replace policy: flexible interface to custom last access time of different types of pages, unified LRU for fair replacement
%     \end{itemize}
%     }
% \end{itemize}
% % \end{itemize}


% \zcsay{extended from Ion's outline (in memory management google doc):)}
% \begin{itemize}
% \item LLM inference workload are memory-bound.
% \item Challenge: 
% \item{\kt{Kuntai Rewrite start}}
% \item{LLM inference workload are quickly growing, and the LLM inference is in general bounded by memory capacity.}
% \item{sdfasdf}
% \item{To alleviate GPU memory pressure, more and more LLMs choose to substitute memory-consuming self-attention to \textit{\textbf{mixing}} different types of attention mechanisms in the same model to handle long context while controlling the size of KV caches (sliding window + self attention), or to handle different types of modalities (self attention + cross attention).}
% \item{Such trend creates new challenges to the memory allocator, as the \textit{\textbf{tensor shape}} and the \textit{\textbf{memory allocation pattern}} are no longer aligned across layers since different layers may use different attention mechanisms.}
% \item{Existing solutions fall short when handling such mix-attention models.}
% \item{Previous work 1: GPU memory virtualization, where the hardware allows a large KV cache tensor to be stored into non-contiguous small pages, but \zc{large malloc overhead, very bad for small models; cross platform support}}
% \item{Previous work 1: PagedAttention, which assumes the memory allocation patterns and the tensor shapes of KV caches are aligned across layers and manage the KV caches on top of this assumption. Advantage: no memory waste when the LLM models only use one types of attention layers across model. Disadvantage: high amount of memory waste when re-purposing it to those models with different types of attentions.}
% \item{Previous work 2: Fix-ratio allcoation (for each types of attention layers, allocate a fixed-size memory pool for its KV cache). This performs well when the size of different types of KV cache size for different layers has a fixed ratio (e.g. }
% \item{\kt{Kuntai rewrite end}}
% \zc{This intro flow only focus on allocation, but prefix caching is also a large part. Should we position prefix caching as a new challenge of the proposed new allocator?}
% \item Inference workloads are growing (maybe give some data that for many users, inference workloads dominate training workloads; probably even for frontier labs, let alone the others)
% % \kt{The sentence is probably a bit too true to feel like i an argument. A possible alternative: LLM inference systems are serving more and more heterogeneous models.}
% \item Despite the increase in the GPU memory over the past 2 years, many inference workloads are still memory bounded \zc{will highlight capacity bound}
% % \kt{After re-read this, this sentence is not spelling out an issue that directly connects to the end-to-end metrics}
% % \kt{Also I heard that the total capacity of HBM manufacturing is bounded, that's probably the main reason of GPU mem}
% \begin{itemize}
%     \item Longer contexts
%     \item MoE model (lower compute density) (\zcsay{we will cover jamba and hunyuan, though no optimization on MoE layer, we can get speedup from larger batch size})
%     \item Large models, e.g., Llama 3 405B
% \end{itemize}

% \item PagedAttention was introduced to address the memory bottleneck by increasing the efficiency of memory allocation, which led to higher throughput and lower costs.
% However, this is no longer enough. Can cite the 78\% memory waste example of mllama.
% \item Why?: Key assumption of PagedAttention: all tokens have the same KV cache size. No longer hold for new models \kt{This sentence is pointing out the phenomena (different tokens have different KV cache sizes) but does not provide a rationale behind it. An example: The key assumption behind PagedAttention is that the attention layers are \textbf{\textit{ homogeneous}} inside the same model, and thus the KV caches has the same shape across different tokens and different layers. However, as more and more techniques are introduced to reduce the KV cache sizes (e.g. sliding window attention, token dropping), or to incorporate with different modalities (e.g. cross attention), the attention layers are becoming more and more \textbf{\textit{heterogeneous}} even inside the same model, resulting in different KV cache sizes for different tokens and layers.} \sout{Models are becoming more complex}  \zc{updated} (e.g.:
%     \begin{itemize}
%         \item multi-modality, different modality may have different number of tokens (mllama, NVLM, flamingo)
%         \item scalable attention techniques like sliding window attention, token drop, \sout{kv cache sharing}
%         \item serving multiple models together (e.g., speculative decoding, LORAs)
%     \end{itemize}
% \item As a result, they require different page sizes, which is a challenge for most memory allocation system
% \item Opportunity: page size are highly aligned ($m\times 2^n$) \kt{There is no direct logic connection between $m\times 2^n$ and we can have practical benefit}, number of different page size is limited. Which is not held in traditional OS memory management
% \item Main idea: two-level allocation, level0 as the lcm of all page size, and some more details. Highlight this is different from OS memory allocation 
% \item Problems
%     \begin{itemize}
%         \item Memory allocation: how to avoid internal fragmentation in level0 page
%         \item Accelerators like GPUs needs regular pages (with only one page size) to execute efficiently
%         \item Cache replacement policies. 1. better cache replacement policies for single type (e.g., for sliding window-based attention) 2. fair replacement policies for different types
%     \end{itemize}
% \item Solutions
%     \begin{itemize}
%         \item Memory allocation: pages of the same request and nearby tokens usually free together or in nearby time step, so we make best effort to let level1 pages in the same level0 page belongs to same request
%         \item Execution: bias based allocation (see Milestone 1 of google doc), need to summarize the high level idea
%         \item Cache replace policy: flexible interface to custom last access time of different types of pages, two-level LRU for fair replacement
%     \end{itemize}
% \item Evaluation shows that xxxx
% \item Contributions: xxx

% page size is not the key problem
% how allocate, how use(todo refine, shared kv), how drop it
% % and 
% % Solution:
% % multiple page sizes
% % Problem: how do you do it so you can limit fragmentation and don’t hurt performance (i.e., access times). 
% % Solution: 
% % Two-level…

% % Somewhere we need to emphasize this is a new memory organization not used before in OSes.

% \end{itemize}

% \zcsay{
% heterogeneous -> token have different types of memory and shapes. \\
% different shape -> allocation fragmentation \\
% different type -> different hit rule \& fair prefix caching


% problem: all three types of work cannot do allocation. Not list related work on prefix caching
% }

% \zcsay{
% we need to design a new memory allocator. 
% It has new challenge in prefix caching.
% Problem: not our sys cause challenge in prefix caching, but heterogeneous
% }


% 8. Insight: empirically, in order to be hardware-compute-friendly, the KV cache size allocation granularity are pre-determined, limited number of types, and  before runtime, and between different layers simultaneously have a very large GCD (2^10) and a relatively small LCM (<10x GCD). 


% 7. However, all possible types of memory are pre-known and the number is limited, so we can partition the memory that compatible to all types, and further partition it as needed. Specifically, LCM, ..., 

% LCM: not need to change kernel

% LCM good: small size is not bottlenecck, allow small fragementation


% Why previous work is not enough: the size ratio between different attention layer's KV caches can be hugely different between requests, but the allocated KV cache space ratio for different attention layers are the same.



% 6. Our insight: previous work has a static mapping between tensor tokens and KV cache addresses

% 6. Our insight: previous work cannot repurposed the same memory for different tokens with different shapes.

% 6. Our insight: the allocation of previous work are fine-grained on tokens but coarse-grained on model layers -- it allocates KV caches for all layers simultaneously

% 6. Our insight: previous work lacks the ability of allocating different size of memory (not fundamental enough)-> due to xxx  LLM's special property, we can do it by xxx.

% 6. all appoaches somehow introduce a fix size, lacks flexibility for allocate different size memory

% 6. All approaches partition the whole memory space into pre-defined static pieces (fixed-size pages in Paged Attention and vAttention, fixed ratio in fixed size partition), and cannot handle the dynamic scenarios where both the size of each components and the memory size ratio of different types of memory are changing.


% Our insight: previous work 


% Goal: we aim to design a memory allocator in LLM inference engines that can serve heterogeneous models with low memory fragmentation.
% \zcsay{then you need to prove we are compatible with ALL inference engine features}

% \kt{
% Flow 2: we aim to design an in-GPU KV cache caching system for heterogeneous models. Challenge:
% 1. cache tensors with different shapes while maximizing memory efficiency
% 2. eviction
% }

% \zcsay{
% \subsection{11/29 Kuntai \& Chen}
% \begin{itemize}
Large language models (LLMs) are becoming popular. Billions of people use ChatGPT~\tocite{}, and millions of people use Github Copilot to write code and documentations~\tocite{}. As a result, the LLM inference workload is rapidly growing. 

However, LLM inference requests are expensive to serve. One single H100 GPU costs \$\tofill{}, and can only fit a medium-size (e.g. Llama 8B) LLM into memory. Also, it takes \tofill{} second to finish processing one request.
The key reason behind such inefficiency is that a single LLM request cannot fully saturate the GPU's parallel computing capability, since LLMs are auto-regressive models that have to generate tokens one-by-one. 

% \zcsay{prefer to simplify this paragraph, just mention it is expensive in one sentence} \kt{I am already reducing the points compared to Ion's outline. Shall we keep simplifying it?}

% Such massive batching challenges the GPU memory management system design, as the KV cache, the intermediate tensors generated by LLM's attention module that can be large, of all requests in the batch needs to be stored on GPU in order to perform batched inference.
% PagedAttention provides a practical solution for those LLMs that only use self-attention attention mechanism, which is a valid assumption for early-stage LLMs.


To accelerate LLM inference, there are two widely-adopted optimizations:
\begin{itemize}
\item \textit{Continuous batching}: Currently-running LLM LLM inference requests can be batched together with new incoming requests to saturate GPU's parallel computing capability. 
\item \textit{Prefix caching}: One can cache the KV Cache (the intermediate tensors generated by LLM's attention layers) of the current request for future use: if a future request share the same prefix with the current request, the KV caches correspond to that prefix can be reused to save GPU computation. 
\end{itemize}
Both optimizations challenge GPU memory management systems. 
Continuous batching requires the memory allocation to lower the GPU memory fragmentation, so that the KV cache of more requests can be kept in GPU and the batch size can be larger.
Prefix caching requires the GPU memory system to store the KV cache of as many frequently-reused prefixes as possible and evict the KV caches when more GPU memory is requires to finish processing the current batch of LLM inference requests.
\zc{simplify this paragraph}

% evict those infrequenly-reused prefixes out from the GPU memory.

% Both of these two techniques challenge the design of GPU memory management system.
% Continuous batching requires the GPU memory management system to store the KV cache of as many requests into GPU as possible to maximally increase the batch size, highlighting the need to an efficient memory allocation module that can allocate GPU memory space of KV caches with low GPU memory fragmentation.
% Prefix caching requires the GPU memory management system to trade between caching the KV caches of one request (so that it can be reused for future request) or discarding the KV cache (to free GPU memory), which requires the GPU memory management to keep frequently-reused KV caches into GPU memory and evict other KV caches from the GPU.




\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/intro-hymba.pdf}
    \caption{LLMs are becoming heterogeneous and produces KV caches with different sizes and life cycles.}
    \label{fig:contrast}
\end{figure}

PagedAttention provides a practical implementation of GPU memory management systems for those LLMs that only use self-attention attention mechanism, which is a valid assumption for early-stage LLMs.
However, LLMs are becoming more and more \textit{\textbf{heterogeneous}}.
Concretely, people will \textbf{\textit{mix}} traditional attention layers \textbf{\textit{together with}} other types of attention layers to customize the model for specific user needs.
For example, \llama 3.2~\cite{dubey2024llama} leverages cross-attention layers for image tokens to handle multi-modality inputs; \gemma~\cite{team2024gemma} leverages sliding window attention layers to better control the KV cache sizes when handling long input context.
\kt{Need some number to let reviewer know that these two types of models are REALLY popular}

We highlight one consequence of such LLM heterogeneity: the KV caches inside one single model will have different sizes and life cycles.
Concretely, as shown in Figure~\ref{fig:contrast}, \mamba \kt{Chen I would recommend using mamba, as 2 types of attention is jsut enough to motivate why the size and the life cycle of KV caches can be different.} \zcsay{I think adding sliding window layer is fine, as we have mentioned sliding window in the previous paragraph. It is good to make it hybrid}
contains two types of the KV caches, where the KV cache for self attention layers need to be always kept in GPU memory when this requrest is in the current batch of LLM inference engine, while the KV cache of Mamba layer is much larger in size but only the KV cache of last token needs to be stored in GPU.
% This also creates new GPU memory saving opportunity for GPU memory management system when it comes to prefix caching.
% For example, if one wants to cache the prefix of the prefix of the current request, it only needs to cache the KV cache for the last token in the prefix for Mamba layers, while for those self attention layers the KV cache for all  tokens need to be cached.

% \kt{Chen can you align the examples}
% \kt{Align the examples and draw figures.}
% \kt{Add more descriptions of the difficulty, and spell out concrete challenges, put prefix caching earlier}
% \kt{WE can be more kind to the reviewers --- heterogeneous memory states, a strawmen solution: static partitioning, obviously bad, dynamically multiplexing, }
% \kt{Chunked prefill -- probably not doable, preemption}

As a result, this paper aims to design the GPU memory management system to maximally utilize GPU memory for heterogeneous LLMs where the KV caches are of different sizes and different life cycles.


One potential solution for this problem is to statically partition the GPU memory into multiple fix-size memory pools, and handle different types of KV caches inside different memory pools.
Such solution works well when the KV cache size ratio between differnet types of attention layers is relatively fixed.
However, this assumption does not hold for \mamba.
This is because that, for self attention layers the KV cache of \textit{all} tokens need to be kept in GPU, but for Mamba layers only the KV cache of \textit{the last} token need to be kept in GPU.
As a result, the size ratio between self-attention KV caches and Mamba KV caches hugely varies when the request lengths are different.
In this scenario, such static partition strategy will result in high GPU memory fragmentation. \zcsay{prefer sliding window here. if not considering prefix caching, fix size partition works well for mamba as mamba cache is very very small.}


Another potential solution is vAttention, where it tailors the GPU memory allocator inside the GPU driver to allocate KV caches with minimum fragmentation.
However, the GPU driver is agnostic to the dependency between KV caches, where we say that KV Cache A depends on KV Cache B, if the KV cache A cannot be reused unless KV cache B is also stored in GPU memory.
For example, as the self attention KV cache of all tokens in the prefix need to be stored in GPU in order to reuse this prefix, the KV cache of all other tokens all depends on the KV cache of the first token. 
If we evict the KV cache of the first token, even if we store the KV cache of all other tokens, that KV cache cannot be reused.
Since such dependency is not visible in the GPU driver, it will wrongfully evict the KV caches that other KV caches depend on, and the other KV caches becomes useless to store in GPU. \zcsay{we can use some figure to explain it}

To conclude, when handling heterogeneous LLMs, previous work either have high GPU memory fragmentation, or waste GPU memory to store KV caches that cannot be reused.

We acknowledge that the general form of such memory management problem (i.e. memory management for different sizes of objects with different life cycles) is indeed extremely challenging and motivates decades of research~\tocite{}.
In LLM applications, however, such problem is much easier to tackle: even though the LLMs can be hugely heterogeneous, the heterogeneity inside one single LLM is relatively limited.
Concretely, we make the following empirical observations:
\begin{itemize}
    % \item The number of different types of KV caches is relatively limited: at most five different types KV caches need to be stored in GPU when serving a LLM. \kt{This argument does not directly motivate the compatibility itself, instead it argues that if we do compatible layer, the overhead is small. So it is probably not a good argument for here.} \cred{VOTE: should we keep this point?}
    \item KV cache sizes inside the same LLM are typically a multiplier of \cred{$2^{10}$} bytes, as this ensures that the computation on top of KV caches can be easily parallelized by the CUDA kernel and among multiple GPUs.
    As a result, it is possible to find a \textit{compatible size}, where not only different types of KV caches can perform memory allocation on top of such compatible size with little internal memory fragmentation, and it allows the GPU memory freed by one types of KV caches can be reused by another.
    % \zc{KV cache sizes inside the same LLM are typically a multiplier of \cred{$2^{10}$} bytes due to the parallelization requirement of GPU architecture. The highly-aligned KV cache size makes compatible page size possible}
   \item Life-cycle-wise, though different types of KV cache can have hugely-different life cycles, these life cycles can be fully determined after specifying the \textit{dependency} between KV caches.
   As a result, we can first implement the API for different types of KV caches to specify the dependencies between tokens and calculate the life cycles for different KV caches, and then implement customized logic to specify the depencendies between KV caches for different types of KV caches.
   % \cred{Current best answer: different types of KV caches all need to customize their prefix caching policy based on the workload to achieve best performance.}
   % \cred{A weaker argument: some KV caches no longer need to be stored in GPU if its dependent KV caches are evicted }
\end{itemize}

\zcsay{some pages need to hit together, challenging to cache system}
\zcsay{the importance of tokens of current request: the longer the important. the importance for future requests: this property not hold (e.g., system prompt, long context qa)}

These observations inspire us to build two-level GPU memory allocator, where the base memory allocator allocates memory using a page size compatible with different KV cache sizes, and the customizable allocators borrow and return memory from the base memory allocator, and executes customized allocation logic to manage the life cycle of different KV caches. 
Based on such insight, we propose \sys, the first GPU memory allocator that maximizes GPU memory utilization for heterogeneous LLMs that uses traditional self-attention together with other types of attentions.
\kt{Chen can you bring in LCM here} \zcsay{Sure, I'll do it tonight. }

To make \sys practical, we further engineer the allocation, caching and eviction logic for a wide range of attention layers, so that it is compatible with a wide range of LLM inference engine optimizations (e.g. speculative decoding and chunked prefill).
% the prefix caching feature of existing LLM inference engines, while making sure that the prefix cache eviction is fair for different types of KV caches. \zcsay{does the discussions before this paragraph include prefix caching? I think including prefix caching like this is quite strange}

% The practical challenge of \sys is: how to support the widely-used prefix caching optimization, so that the KV caches computed by one request can be reused by another request with the same prefix?
% To handle this challenge, we engineer the allocation, caching and eviction logic for a wide range of attention layers, so that it is compatible with the prefix caching feature of existing LLM inference engines, while making sure that the prefix cache eviction is fair for different types of KV caches. \zcsay{does the discussions before this paragraph include prefix caching? I think including prefix caching like this is quite strange}

We evaluate on \sys on \tofill{} LLMs, \tofill{} datasets and \tofill{} GPUs. Our evaluation shows that, compared to state-of-the-art LLM serving engine vLLM, \sys achieves \tofill{}x higher throughput without hurting the end-to-end latency, by maximally batching LLM inference requests with little memory waste. Also, \sys is significant under different GPUs. \sys is also compatible with a wide range of features in LLM serving engines.

To summarize, the contribution of this paper is as follows:
\begin{packeditemize}
    \item A GPU memory allocator that improves throughput for those LLMs with differet KV cache sizes and life cycles, by maximally batch requests with minimum GPU memory waste. \zcsay{add also clever prefix caching?}
    \item A practical implementation, \sys, that is implemented on top of production-level inference engine vLLM and is compatible to a wide range of inference engine features.
    \item \sys improves the serving engine throughput by \tofill{}$\times$ without sacrificing request serving latency.
\end{packeditemize}

% \item Practical problems
%     \begin{itemize}
%         \item Memory allocation: how to avoid internal fragmentation in large page
%         \item Accelerators like GPUs needs regular pages (with only one page size) to execute efficiently, but we have multiple page sizes now
%         \item Allow each type to customize cache management strategy flexibly % Cache replacement policies. ) 2. fair replacement policies for different types
%     \end{itemize}
% \item Solutions
%     \begin{itemize}
%         \item Memory allocation: request-aware allocation to avoid internal fragmentation
%         \item Execution: represent the allocation result of each layer as single-size pages, with minimal changes to the workers
%         \item Cache replace policy: flexible interface to custom last access time of different types of pages %, unified LRU for fair replacement
%     \end{itemize}
% \end{itemize}

% \zc{show new eviction policy as our contribution}

% \kt{
% 7. Two functionalities: 1. which memory need to be allocated (allocation) 2. what should be the type of that allocated memory (instantiation)
% We argue that, we should decouple these two dec
% which memory need to be allocated to what type.
% We argue that we should implement \textit{multiple} memory allocators to allow the allocation / free of different types to decouple with other types, while these multiple memory allocators need 
% }


% 1) which memory should be allocated to which type
% 2) how to use this piece of memory

% how to customize the allocate / \cred{access, need replace} /free patterns of the heterogeneous types, while allowing these customized memory access patterns compatible with each other

% how to customized the usage of memory of hetergeneous type, while allowing these things to exchange memory with each other as needed.

% \item We argue for a \textit{two-layer} desi

% \item Insight: we design a new that can be repurposed 
% \item then, two questions: 1) how to express the unique memory patterns of different component 2) how to fairly and efficiently distributed the overall memory resource to different types

% \subsection{12/03 Woosuk}



==> intro_v5.tex <==
\section{12/08 Woosuk Intro}

Recent advancements in AI have fueled the ambition to develop more capable and versatile models that can perceive images, process audio, and understand very long documents.
This has sparked a new paradigm where large language models (LLMs) incorporate \textit{heterogeneous} components within a single architecture, moving beyond the limitations of monolithic Transformers~\cite{vaswani2017attention}.
These components include neural networks to process diverse modalities—such as vision encoders for images and audio encoders for sound—as well as variants of attention algorithm~\cite{beltagy2020longformer,gu2023mamba} for handling long-context inputs.

These diverse components introduce heterogeneous states, or \textit{embeddings}, during inference of the model.
For example, the PaliGemma 2~\cite{steiner2024paligemma2familyversatile} vision-language model (VLM) first projects the image inputs to \textit{vision embeddings}, a set of embedding vectors representing the images.
Next, the vision embeddings and text inputs are consumed by the LLM backbone, Gemma 2~\cite{team2024gemma}, which interleaves global attention and sliding window attention~\cite{beltagy2020longformer} to efficiently support long-context inputs.
Gemma 2 produces two types of embeddings from the inputs, namely KV cache~\cite{} for global attention layers and another KV cache for sliding window attention layers.
While the model generates the output, these embeddings need to be stored in GPU memory.

Managing these heterogeneous states poses a new challenge in serving LLMs.
The throughput of LLM serving is typically memory capacity-bound~\cite{kwon2023efficient}; Inefficient use of GPU memory could limit the number of requests that can be batched and processed in parallel, and thereby limit the GPU utilization.
While PagedAttention~\cite{kwon2023efficient} was introduced to efficiently manage the KV cache for global attention, it fails to do so when multiple types of embeddings co-exist in the same model.
We find two reasons for this:

First, different types of embeddings often have different sizes.
For instance, the size of the vision embedding of an image patch can be larger than that of the KV cache corresponding to a text token~\cite{dubey2024llama}.
Importantly, this violates a key assumption in PagedAttention that the memory space can be partitioned with a single embedding size.
As different types of embeddings have to dynamically share the GPU memory space, the different sizes can lead to significant memory fragmentation if not handled properly.

Second, different types of embeddings can have different life cycles.
For example, in the global attention layers of Gemma 2, the KV cache of all previous tokens is needed to generate the next token.
On the other hand, in its sliding window attention layers, only the KV cache of the most recently generated tokens is needed, allowing the embeddings of the other tokens to be 
This difference complicates determining which embedding to evict.

State-of-the-art LLM inference engines~\cite{kwon2023efficient,trtllm,zheng2023efficiently} struggle with 

% One approach to this problem, which is employed by state-of-the-art LLM inference engines such as vLLM~\cite{kwon2023efficient}, is to ignore the different characteristics of the heterogeneous embeddings and treat them as homogeneous ones.
% For example, vLLM unifies different embedding sizes through padding, and treats sliding window attention as like global attention, retaining all embeddings 


\subsection{12/05 Woosuk Outline}

1. People want more capable AI, seeing images, listening to audios, and understanding very long documents. This has sparked a new paradigm where LLMs include heterogeneous components in a single model.
  * NNs to process different modalities (vision encoder, audio encoder, etc.)
  * Efficient algorithms to cover long context inputs

2. Different components produce heterogeneous memory states ("embeddings") at the inference time.
  * PaliGemma2 model as a running example
  * image embeddings produced by the encoders
  * normal KV caches
  * KV cache variants (sliding window, mamba)
  * + audio/video **in a single model** in the future (GPT-4o, Gemini)

3. Managing these memory states poses a new challenge in serving LLMs: We found that while PagedAttention works greatly on normal KV caches, it fails in efficiently managing these heterogeneous states. We found two problems:

4. First, different states can have different embedding sizes. For example, ... .

5. Second, different memory states have different lifecycles and access patterns. When the GPU memory is full, the system needs to evict some embeddings to accommodate the embeddings of the newly generated tokens. While normal attention assumes that all previous embeddings are needed to generate the next token, this is not the case for other variants. For example, in sliding window attention, only the most recently generated tokens are accessed.

6. This is a challenging problem because these heterogeneous memory states in different layers have dependencies between each other. For example (PaliGemma2?), where one request can have image embeddings, global attention KV cache, and sliding window KV cache, . For the model to generate the next token,  

7. One approach to this problem, which is employed by popular LLM inference engines such as vLLM~\cite{}, is to ignore the different characteristics of the heterogeneous embeddings and treat them as homogeneous ones. For example, vLLM unifies the different embedding sizes by padding them. Also, vLLM treats sliding window attention as like global attention, keeping the embeddings of all the prior tokens even though only the recent ones are used in sliding window attention. As a result, it has significant memory waste.

8. Another possible approach is to implement a sophisticated memory allocator that takes embedding sizes, access patterns, inter-layer dependencies as inputs, and makes global memory allocation/eviction decisions for all types of embeddings. Unfortunately, however, this would make the memory allocator too complex and difficult to scale. Many different combinations of embeddings + new modalities and algorithms are consistently added.
If not handled properly, this can lead to significant memory fragmentation. "Memory fragmentation reduces the number of requests that can be concurrently processed by the serving system, severely limiting the performance (cite PagedAttention)"
 
9. In this paper, we propose \sys, an efficient and customizable memory allocator for heterogeneous embeddings in LLM inference. In contrast to the monolithic memory allocator in existing systems~\cite{}, \sys introduces \textit{two-level memory management}, which consists of a generic large-memory allocator and customized small-memory allocators for different types of embeddings. \sys provides APIs for the small-memory allocators to express the size and access pattern of each type of embedding in the model. Then, the large-memory allocator serves as a compatibility layer that dependency . This design enables supporting many different combinations of embeddings that could co-exist in the same model, without increasing the complexity.

10. To mitigate the internal fragmentation due to different embedding sizes, \sys's large-memory allocator allocates large pages whose size is the \textit{least common multiplier} (LCM) of every embedding size in the model.
Then, ...
While this approach could theoretically lead to significant memory fragmentation when the LCM is excessively large, we find that this scenario is rare in practice. As shown in~\ref{}\woosuk{We need a table in sec 4}, the embedding sizes in production-level LLMs are typically expressed in the form $n \cdot 2^k$ where $n$ is a small integer (less than 10), and therefore their LCM remains relatively small.
This pattern is not coincidental; it reflects the design of AI accelerators, such as GPUs and TPUs, which work best when embedding sizes align with powers of two. 

11. 

12. We have implemented \sys on top of vLLM. Thanks to its modular design, \sys can support a wide variety of models with heterogeneous embeddings. Furthermore, thanks to the LCM-based memory allocation, \sys does not require any modification to the existing GPU kernels~\cite{}, which is expensive to modify.
In our experiments, \sys improves the LLM serving throughput by $\times$ on average and up to $\times$, by reducing the memory fragmentation by $\times$.

\subsection{Introduction}


% \begin{itemize}
%     \item PagedAttention was great, blah, blah...
%     \item However, PagedAttention makes to (implicit) assumptions (1) all embeddings have the same size and (2) all the prefix is required to general the next tokens. This informs memory management including eviction algorithms.
%     \item However, the new LLMs architectures are becoming far more heterogeneous and are braking these two assumptions.
%     \item One para size
%     \item One para what tokens you need in memory
% \end{itemize}


% {Ion's Proposed Flow:
% \begin{itemize}
% \item LLMs are changing the world.
% \item LLM inference is growing in importance due to the generality of LLMs (i.e., you don't need to train them for each task) and test-time inference/compute.
% \item LLM inference is hugely expensive; making it efficient is the key.
% \item (Remind people how did we get to vLLM) Token generation is sequential $\rightarrow$ batches to improve parallelism but memory becomes a bottleneck $\rightarrow$ page attention to improve memory utilization and increase batch size.
% \item Many things have changed since PagedAttention has been introduced (e.g., multi-modal models, mixed state-space, etc) $\rightarrow$ The result: we need to support multiple embedding sizes. 
% \item So key challenge is to support multiple embedding sizes and maximize mem utilization. One solution is to have larger page sizes but can lead to internal fragmentation.  
% \item Our solution: two-level memory management based on LCM.
% \item Also heterogeneity brings new (fundamental) challenges to how we do eviction, caching.
% \item ...
% \end{itemize}
% }

% \zcsay{Ion says hetogeneous only related to the size but may be ok}
% \zcsay{prefer remove token de. woosuk: add co-exist in Ion's flow}

% \subsection{Kuntai's version}
% \woosuk{I think the current flow has too many hops. Why don't we start from directly pointing out the difficulty of managing heterogeneous memory states?
% Also, I think we should not focus too much on fragmentation and memory waste, since it does not include prefix caching for heterogeneous layers.}

% Large language models (LLMs) are becoming more and more popular. Billions of people use ChatGPT~\tocite{}, and millions of people use Github Copilot to write code and documentations~\tocite{}.
% To handle huge LLM workload, people find that it is crucial to enlarge LLM inference \textit{batch size}, which allows more requests to be processed within single LLM forwarding pass while only marginally increase the LLM forwarding latency~\tocite{}. \zhuohan{Why talk about batch size here? I feel the concept of batch size comes out of the blue and seems unnecessary here.} \zcsay{we need to point out why avoiding memory waste is important}
% % without  is to perform LLM inference with as large batch size as possible, so that 
% % maximally enlarge the LLM inference batch size, by designing a GPU memory allocator that can fit as many requests into the GPU memory as the GPU memory permits.
% Based on such insight, people develop LLM inference engines (e.g., vLLM~\tocite{} and TGI~\tocite{}) that maximally increase the batch size (by using customized GPU memory allocator to fit as many requests into GPU memory as possible) and thus serve LLM inference requests with much high throughput without inflating the end-to-end latency.

% % \zcsay{We need to highlight batch size is important here, instead of saying "they have good batch size".}
% % \kt{My feeling is that we need to spend a lot of text in intro if we want to explain why large batch size leads to higher throughput (and this text does not really push the logic forward). }
% % Let me try: Due to the xxx property of LLM serving, the throughput of these inference engines highly depends on the number of LLM inference requests that can be batched together, so they design memory allocators to maximally batches as many LLM inference requests as the GPU memory permits}


% Alongside the significant rise of LLM inference workloads, LLM architectures also get increasingly \textit{heterogeneous}, where LLMs use traditional attention layers \textbf{\textit{together with}} other types of attention layer to better customize the model for specific user needs, while maximally preserving the accuracy of the models. 
% For example, \llama 3.2~\cite{dubey2024llama} leverages cross-attention layers for image tokens to handle multi-modality inputs; \gemma~\cite{team2024gemma} leverages sliding window attention layer to better control the KV cache sizes when handling long input context.
% % , or representing all historical information into a very large but fixed size of tensor (e.g. mamba)
% Such heterogeneous attention layers also generate KV caches (the intermediate data of attention layers that need to be cached to generate new tokens) with \textit{different KV cache granularities} (we define the KV cache granularity as the KV cache size for one single token) and \textit{for different sets of tokens}.

% % For example, \llama 3.2 generates KV cache for image tokens and text tokens seperately, where the KV cache granularity for each text token is $4\times$ larger than that of image tokens. 

% As a result, the research question of this paper is: How to design a GPU memory allocator for LLM inference engines that allows maximum batch size for heterogeneous LLM architectures by allocating KV caches with minimum GPU memory fragmentation?

% % There are three types of prior work that handles this challenge, but they all introduces significant memory waste. \zcsay{Related work part is a little long, is it possible to only discuss paged attention here, and put other parts in a seperate discussion section?}

% Existing inference engines tackle this research question by PagedAttention.
% The key innovations of PagedAttention is that it allows partitioning the KV caches generated by LLMs along token dimensions and store each piece of partitioned KV cache into non-adjacent GPU memory addresses, with minimum impact on LLM inference performance.
% % Concretely, it calculates the amount of GPU memory consumed by LLM when handling a fixed amount of tokens (by default 16 in vLLM), and then partitions the GPU memory into pages using such value.
% Such PagedAttention-based inference engines has very low GPU memory fragmentation when handling those models that only uses one type of attention layers.
% However, PagedAttention has significant GPU memory fragmentation when supporting LLMs that use different types of attention layers.
% Concretely \kt{Quantify the amount of memory waste here} %\zcsay{TODO: show the memory waste calculated in sec 3}.

% The key reason behind such GPU memory fragmentation is that PagedAttention's GPU memory allocation strategy is \textit{agnostic} to different types of attention layers, resulting in fixed GPU memory allocation ratio between different attention layer types.
% However, the ratio between the actual GPU memory required by the KV cache of different attention layer types \textit{hugely varies} between different batches.
% \kt{Quantify how much such allocation ratio can vary.}
% As a result, the GPU memory fragmentation can be substantial when the fixed allocation ratio significantly mismatches the actual ratio for the current batch.

% % approaches shares the same limitation: they all partition the whole memory space into pre-defined static pieces (fixed-size pages in Paged Attention and vAttention, fixed ratio in fixed size partition), but the optimal KV cache size partition for different attention layers hugely depends on the context length, and thus vary a lot between different batches.

% % The second type of work is vAttention that allows the LLM applications to allocate large tensors, while the under GPU driver partitions the tensor into small pages (each page is of size 64KB) and performs memory allocation based on such small pages. 
% % This design offloads the memory allocation complexity to GPU drivers, which introduces much higher engineering overhead compared to performing memory allocation inside LLM serving engines, as GPU drivers are much difficult to program, and the effort of changing the driver cannot be reused by other types of GPUs. \zcsay{not true, discussion needed}

% % The third type of work is creating a fix-size memory pool for different types of KV caches, and then perform memory allocation inside each pool. 
% % As a result, the GPU memory allocation ratio between different types of attention layers are fixed, and result in high memory waste when serving models with different types of attentions.

% We argue that: instead of fixing the ratio of GPU memory size between different types of attention layers, the memory allocator needs to be able to \textbf{\textit{dynamically}} adjust such ratio to match the actual GPU memory requirement ratio of the current LLM inference batch.

% Such dynamic memory allocation is in general difficult and motivates decades of research~\tocite{}.
% However, in LLM applications, such problem is much simpler to tackle: though different LLMs have highly heterogeneous attention layers, empirically we observe that the heterogeneity inside the same LLM is much more \textbf{\textit{limited}}. 
% Concretely, a typical LLM uses at most 3 different types of attention layers, and the size of those KV caches are typically a multiplier of $2^{10}$ bytes, in order to maximize the hardware computation efficiency. \kt{Chen please update these numbers}.
% This inspires us to create a \textit{compatibility layer} that can be dynamically allocated and used for any kind of KV caches inside the same LLM.


% A naive approach of building such compatibility layer is to partition the GPU memory into pages, where the page size is the greatest common denominator (GCD) for different types of KV caches. We then build memory allocators for different types of attention layers on top of the compatibility layers.
% However, this solution significantly slows down the LLM inference engine.
% This is because most-performant GPU kernels typically requires the KV cache to be contiguous alongside several tensor dimensions, and the GCD solution may have to partition the tensor along that dimension. As a result, people need to customize GPU kernels for a wide range of possible GCDs, which significantly increasing the GPU kernel engineering overhead and still the performance will not match those most-performant GPU kernels. 

% % Also these GPU kernels also significantly inflates the package size \zcsay{can others know what is ``package size''?} of inference engine, slowing down the development and deployment of inference engines.


% In contrast, we build such compatibility layer by partitioning the GPU memory into large pages with the page size as the lowest common multiplier (LCM) of different KV cache allocation granularity.
% We then build different GPU memory allocators for different types of KV caches, where these memory allocators dynamically adjust the GPU memory pool size by allocating / freeing the large pages, and then perform allocation inside their GPU pool.
% Such a solution ensures that the KV cache allocation granularity is always a multiplier of the KV cache allocation granularity of existing inference engines, and thus are compatible with the GPU kernels of existing engines.

% We build \sys, the first system that allocates GPU memory for LLM applications, by layering the memory allocator into \textit{compatibility layer} using the LCM of different KV cache allocation granularities, and then build \textit{attention-aware} layer that allocates GPU memory on top of them. \zcsay{compatibility layer vs model layer. a little confusing, better to choose another name}

% To make \sys practical, we design the algorithm of \tofill{} to minimizes the internel fragmentation (Section ??) and make sure it is compatible with the prefix caching feature in LLM inference engines (Section ??). \zcsay{the space left for prefix caching is too short. Memory management includes allocation and caching, I think we can discuss caching very fluently in intro.} \kt{Let's discuss and figure out the flow to discuss prefix caching}

% \zc{Evaluation shows that \sys can improve the maximum batch size by \tofill{} times and improve the serving throughput by \tofill{} times on average on a set of heterogeneous LLMs.}% \kt{Chen please add placeholders here}
% % \zcsay{will fill in the last day}

% To summarize, the contributions of this paper are:
% \begin{itemize}
%     \item A GPU memory allocator that minimizes GPU memory fragmentation for those models with heterogeneous attention layers.
%     \item A practical implementation, \sys, that is implemented on top of production-level inference engine vLLM and is compatible to a wide range of inference engine features.
%     \item \sys improves the serving engine throughput by ??$\times$ without sacrificing request serving latency.
% \end{itemize}

% \subsection{Zhuohan's version}
% \begin{itemize}
%     \item \zc{still need: LLM is popular, LLM memory management is important}
%     \item Memory management for LLMs are becoming more complicated than before (when vLLM just came out)
%     \begin{itemize}
%         \item Models become more complicated:
%             \begin{itemize}
%                 \item Sparse attention layers: sliding window/pyramid kv
%                 \item Mixed with state-space model: Jamba
%                 \item Multi-modality: llava and llama
%                 \item Layer sharing (not sure whether this is challenging for existing memory management scheme) \zcsay{prefer not to discuss  layer sharing in this paper, as it is still fixed size pages}
%             \end{itemize}
%         \item LLM inference optimizations also bring challenges to the memory manager
%         \begin{itemize}
%             \item Spec decode (need to manage small model's memory)
%             \item Prefix caching (how to free kv cache across different layers?)  \zcsay{Prefix caching is much more important than a sub-sub item in paper flow, needs a fluent way to bring it in, but still keep the two-level allocation as the major contribution that we want the readers to remember}
%         \end{itemize}
%         \item All of above make managing LLM's runtime memory beyond managing a bunch of fixed size pages, which is the main challenge of this paper.
%     \end{itemize}
%     \item 
%     \kt{We probably need to bring in some related work here}
%     \zcsay{Prefer to discuss about the unique properties in LLM that leads to a different design with traditional OS, which is our main insight}
%         \item Our major technique: Hierarchical memory allocation to handle \zcsay{I like Kuntai's statements on compatibility layer and re-purposing}
%         \begin{itemize}
%             \item Specifically, two level: Large page and small page.
%                 \item Large page for functionality xxx, small pages for functionality yyy.
%                 \item Large pages takes an LCM of sizes of small pages (please don't highlight this that much in the intro. I think this is pretty straight forward)
%     \end{itemize}
%     \item Some supporting techniques (I don't fully understand this at the moment and we can discuss more tmrw)
%     \begin{itemize}
%         \item Request Aware Allocation to Reduce Internal Fragmentation (I don't understand this part fully)
%         \item Layer grouping (can be discussed together with layer sharing)
%         \item Prefix caching support (need to highlight some techniques here).
%     \end{itemize}
%     \item \zcsay{I like my previous version on supporting techniques part:}
%    \zc{ \item Problems
%     \begin{itemize}
%         \item Memory allocation: how to avoid internal fragmentation in large page
%         \item Accelerators like GPUs needs regular pages (with only one page size) to execute efficiently, but we have multiple page sizes now
%         \item Cache replacement policies. 1. better cache replacement policies for single type (e.g., for sliding window-based attention) 2. fair replacement policies for different types
%     \end{itemize}
% \item Solutions
%     \begin{itemize}
%         \item Memory allocation: request-aware allocation to avoid internal fragmentation
%         \item Execution: represent the allocation result of each layer as single-size pages, with minimal changes to the workers
%         \item Cache replace policy: flexible interface to custom last access time of different types of pages, unified LRU for fair replacement
%     \end{itemize}
%     }
% \end{itemize}
% % \end{itemize}


% \zcsay{extended from Ion's outline (in memory management google doc):)}
% \begin{itemize}
% \item LLM inference workload are memory-bound.
% \item Challenge: 
% \item{\kt{Kuntai Rewrite start}}
% \item{LLM inference workload are quickly growing, and the LLM inference is in general bounded by memory capacity.}
% \item{sdfasdf}
% \item{To alleviate GPU memory pressure, more and more LLMs choose to substitute memory-consuming self-attention to \textit{\textbf{mixing}} different types of attention mechanisms in the same model to handle long context while controlling the size of KV caches (sliding window + self attention), or to handle different types of modalities (self attention + cross attention).}
% \item{Such trend creates new challenges to the memory allocator, as the \textit{\textbf{tensor shape}} and the \textit{\textbf{memory allocation pattern}} are no longer aligned across layers since different layers may use different attention mechanisms.}
% \item{Existing solutions fall short when handling such mix-attention models.}
% \item{Previous work 1: GPU memory virtualization, where the hardware allows a large KV cache tensor to be stored into non-contiguous small pages, but \zc{large malloc overhead, very bad for small models; cross platform support}}
% \item{Previous work 1: PagedAttention, which assumes the memory allocation patterns and the tensor shapes of KV caches are aligned across layers and manage the KV caches on top of this assumption. Advantage: no memory waste when the LLM models only use one types of attention layers across model. Disadvantage: high amount of memory waste when re-purposing it to those models with different types of attentions.}
% \item{Previous work 2: Fix-ratio allcoation (for each types of attention layers, allocate a fixed-size memory pool for its KV cache). This performs well when the size of different types of KV cache size for different layers has a fixed ratio (e.g. }
% \item{\kt{Kuntai rewrite end}}
% \zc{This intro flow only focus on allocation, but prefix caching is also a large part. Should we position prefix caching as a new challenge of the proposed new allocator?}
% \item Inference workloads are growing (maybe give some data that for many users, inference workloads dominate training workloads; probably even for frontier labs, let alone the others)
% % \kt{The sentence is probably a bit too true to feel like i an argument. A possible alternative: LLM inference systems are serving more and more heterogeneous models.}
% \item Despite the increase in the GPU memory over the past 2 years, many inference workloads are still memory bounded \zc{will highlight capacity bound}
% % \kt{After re-read this, this sentence is not spelling out an issue that directly connects to the end-to-end metrics}
% % \kt{Also I heard that the total capacity of HBM manufacturing is bounded, that's probably the main reason of GPU mem}
% \begin{itemize}
%     \item Longer contexts
%     \item MoE model (lower compute density) (\zcsay{we will cover jamba and hunyuan, though no optimization on MoE layer, we can get speedup from larger batch size})
%     \item Large models, e.g., Llama 3 405B
% \end{itemize}

% \item PagedAttention was introduced to address the memory bottleneck by increasing the efficiency of memory allocation, which led to higher throughput and lower costs.
% However, this is no longer enough. Can cite the 78\% memory waste example of mllama.
% \item Why?: Key assumption of PagedAttention: all tokens have the same KV cache size. No longer hold for new models \kt{This sentence is pointing out the phenomena (different tokens have different KV cache sizes) but does not provide a rationale behind it. An example: The key assumption behind PagedAttention is that the attention layers are \textbf{\textit{ homogeneous}} inside the same model, and thus the KV caches has the same shape across different tokens and different layers. However, as more and more techniques are introduced to reduce the KV cache sizes (e.g. sliding window attention, token dropping), or to incorporate with different modalities (e.g. cross attention), the attention layers are becoming more and more \textbf{\textit{heterogeneous}} even inside the same model, resulting in different KV cache sizes for different tokens and layers.} \sout{Models are becoming more complex}  \zc{updated} (e.g.:
%     \begin{itemize}
%         \item multi-modality, different modality may have different number of tokens (mllama, NVLM, flamingo)
%         \item scalable attention techniques like sliding window attention, token drop, \sout{kv cache sharing}
%         \item serving multiple models together (e.g., speculative decoding, LORAs)
%     \end{itemize}
% \item As a result, they require different page sizes, which is a challenge for most memory allocation system
% \item Opportunity: page size are highly aligned ($m\times 2^n$) \kt{There is no direct logic connection between $m\times 2^n$ and we can have practical benefit}, number of different page size is limited. Which is not held in traditional OS memory management
% \item Main idea: two-level allocation, level0 as the lcm of all page size, and some more details. Highlight this is different from OS memory allocation 
% \item Problems
%     \begin{itemize}
%         \item Memory allocation: how to avoid internal fragmentation in level0 page
%         \item Accelerators like GPUs needs regular pages (with only one page size) to execute efficiently
%         \item Cache replacement policies. 1. better cache replacement policies for single type (e.g., for sliding window-based attention) 2. fair replacement policies for different types
%     \end{itemize}
% \item Solutions
%     \begin{itemize}
%         \item Memory allocation: pages of the same request and nearby tokens usually free together or in nearby time step, so we make best effort to let level1 pages in the same level0 page belongs to same request
%         \item Execution: bias based allocation (see Milestone 1 of google doc), need to summarize the high level idea
%         \item Cache replace policy: flexible interface to custom last access time of different types of pages, two-level LRU for fair replacement
%     \end{itemize}
% \item Evaluation shows that xxxx
% \item Contributions: xxx

% page size is not the key problem
% how allocate, how use(todo refine, shared kv), how drop it
% % and 
% % Solution:
% % multiple page sizes
% % Problem: how do you do it so you can limit fragmentation and don’t hurt performance (i.e., access times). 
% % Solution: 
% % Two-level…

% % Somewhere we need to emphasize this is a new memory organization not used before in OSes.

% \end{itemize}

% \zcsay{
% heterogeneous -> token have different types of memory and shapes. \\
% different shape -> allocation fragmentation \\
% different type -> different hit rule \& fair prefix caching


% problem: all three types of work cannot do allocation. Not list related work on prefix caching
% }

% \zcsay{
% we need to design a new memory allocator. 
% It has new challenge in prefix caching.
% Problem: not our sys cause challenge in prefix caching, but heterogeneous
% }


% 8. Insight: empirically, in order to be hardware-compute-friendly, the KV cache size allocation granularity are pre-determined, limited number of types, and  before runtime, and between different layers simultaneously have a very large GCD (2^10) and a relatively small LCM (<10x GCD). 


% 7. However, all possible types of memory are pre-known and the number is limited, so we can partition the memory that compatible to all types, and further partition it as needed. Specifically, LCM, ..., 

% LCM: not need to change kernel

% LCM good: small size is not bottlenecck, allow small fragementation


% Why previous work is not enough: the size ratio between different attention layer's KV caches can be hugely different between requests, but the allocated KV cache space ratio for different attention layers are the same.



% 6. Our insight: previous work has a static mapping between tensor tokens and KV cache addresses

% 6. Our insight: previous work cannot repurposed the same memory for different tokens with different shapes.

% 6. Our insight: the allocation of previous work are fine-grained on tokens but coarse-grained on model layers -- it allocates KV caches for all layers simultaneously

% 6. Our insight: previous work lacks the ability of allocating different size of memory (not fundamental enough)-> due to xxx  LLM's special property, we can do it by xxx.

% 6. all appoaches somehow introduce a fix size, lacks flexibility for allocate different size memory

% 6. All approaches partition the whole memory space into pre-defined static pieces (fixed-size pages in Paged Attention and vAttention, fixed ratio in fixed size partition), and cannot handle the dynamic scenarios where both the size of each components and the memory size ratio of different types of memory are changing.


% Our insight: previous work 


% Goal: we aim to design a memory allocator in LLM inference engines that can serve heterogeneous models with low memory fragmentation.
% \zcsay{then you need to prove we are compatible with ALL inference engine features}

% \kt{
% Flow 2: we aim to design an in-GPU KV cache caching system for heterogeneous models. Challenge:
% 1. cache tensors with different shapes while maximizing memory efficiency
% 2. eviction
% }

% \zcsay{
% \subsection{11/29 Kuntai \& Chen}
% \begin{itemize}

Large language models (LLMs) have become increasingly popular across a wide range of applications. 
Tools like ChatGPT~\tocite{} have reached hundreds of millions of users, while platforms such as GitHub Copilot assist millions of people with intelligent code completion~\tocite{}. 
Such rapid growth in LLM adoption has significantly increased the LLM inference workload.

Serving LLM inference requests, however, is expensive. One single H100 GPU costs approximately \$5 per hour but can only accommodate a medium-size model (e.g., Llama 8B) in GPU memory. Moreover, processing a single request on such top-tier GPU can take up to 31 seconds. \ps{Better give the number for a typical size of request.} \zcsay{we focus on throughput, throughput data may be better than latency}



GPU memory management is important in improving LLM inference efficiency. Concretely, previous work PagedAttention~\tocite{} shows that KV caches (intermediate tensors generated by the attention module and stored in GPU memory for inference) can be managed token-by-token. 
Thenrfore, it splits GPU memory into \textbf{\textit{fixed-size pages}}, where the page size is the KV cache size of one token, and allocates/frees KV caches at page granularity to GPU memory fragmentation and improve GPU memory utilization. 
Empirically, this optimization increases memory utilization by $3.59\times$, allowing larger batching during inference and improving LLM serving throughput by 2–4$\times$. 
Additionally, PagedAttention enables \textbf{\textit{prefix caching}}, allowing future request to reuse the KV cache of the current request if they have shared prefix.
This further reduces redundant computation and accelerates applications like long-document question answering by up to 5$\times$. \ps{I think you don't need to discuss the benefits of paged attention this early in the intro?}


The success of PagedAttention implicitly relies on two assumptions that hold for most early-stage LLMs, which typically consist of stacked self-attention layers: 
\begin{itemize}
    \item \textbf{Uniform granularity}: KV caches have the same size across different tokens and layers. We refer to this size as the \textit{granularity} of KV cache. 
    This property allows the GPU memory management system to manage the KV cache of the whole LLM using one  granularity.
    \item \textbf{Prefix dependency}: The KV caches of all prefix tokens need to be stored in GPU in order to generate a new token. This is also required for the prefix cache to be reused by future requests.  \ps{Is this an assumption of page attention? it can do block sparsity, right?}
\end{itemize}

% However, LLMs are becoming more and more \textit{\textbf{heterogeneous}} and break these two assumptions.
However, frontier LLMs are becoming increasingly \textit{\textbf{heterogeneous}}, combining self-attention with special types of attention mechanisms inside the same model for specific user needs. \ps{would be good to get to the problem earlier. someone else thinks that ``I think you don't need to discuss the benefits of paged attention this early in the intro''} \zcsay{We should use Woosuk's flow that first talk about heterogeneous and then talk about pagedattention}
For example, \llama 3.2~\cite{dubey2024llama} from Meta leverages cross-attention layers to handle multi-modality inputs; \gemma~\cite{team2024gemma} from Google uses sliding window attention layers to reduce KV cache sizes for long-context inputs. \ps{This feels a bit limited to these two models but your technique is much more general. Maybe start with "multi-modality layers" and "sliding window layers" to emphysize layer heterogeneity and use models as examples that adopt these hetrogenous layers.}
Both LLMs are widely adopted in industry and empower a bunch of production services.\ps{need example} \zcsay{tried to find some example, but failed.}

These heterogeneous LLMs violates the assumptions of uniform granularity and prefix dependency:



\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/intro-hymba.pdf}
    \caption{LLMs are becoming heterogeneous and produces KV caches with different sizes and life cycles.}
    \label{fig:contrast}
\end{figure}


First, the KV caches inside one model can have different granularities.
For example, NVIDIA's Hymba model~\tocite{} combines self attention layers, sliding window attention layers and mamba layers to further save the KV cache memory footprint than \gemma, as shown in Figure~\ref{fig:contrast}.
The KV cache of Mamba layer has much larger granularity \ps{What do you mean by larger granularity ? might be good to explain for general systems community.} \zcsay{we may change granularity to some direct word like embedding size} that allows LLM to store more information in the KV cache than the other two types.


Second, the dependency rules also vary across layers. \ps{The wording "rule" is a bit weird}
While self-attention layers retain KV caches for all prefix tokens, sliding-window layers only require storing the KV cache for the most recent tokens within the sliding window, and Mamba layers depend solely on the KV cache of the last token.

% Concretely, in Hymba model, though self attention layers are prefix-dependent and the KV cache of all prefix tokens need to be stored in order to generate new token, but we only need to keep the KV cache inside the sliding window for sliding window layer, and of the last token for Mamba layer.

% \sout{Though we only use Hymba in the above example, the violation of these two assumptions widely exist. See \S\tofill{} for more details.}

% The KV cache of Mamba layer will be much larger in size compared to self attention layer and lsbut only the KV cache of last token needs to be stored in GPU.
% Concretely, the KV cache of sliding windows layers have the same size per token as the traditional self attention layers but we only need to keep the KV cache inside the sliding window.


% meta-released \llama 3.2~\cite{dubey2024llama} leverages cross-attention layers for image tokens to handle multi-modality inputs; 
% Google-released \gemma~\cite{team2024gemma} leverages sliding window attention layers to reduce KV cache sizes when handling long input context;
% NVIDIA-released \hymba leverages mamba layers that condenses the context into a large tensor with fix size to 
% \kt{Need some number to let reviewer know that these two types of models are REALLY popular}
% Both models break the two assumptions 

% The performance cost of breaking these two assumptions is prohibitive.
% We measure the GPU memory fragmentation in vLLM, a production-level LLM inference engine that uses PagedAttention to manage the GPU memory, and found that over \tofill{} of GPU memory are wasted when serving \tofill{} models, leading to \tofill{} throughput degradation.
% Furthermore, the prefix caching support is still broken, despite that this LLM has already been released for \tofill{} months. \todo{cannot list number like this}





% Such LLM heterogeneity will the KV caches inside one single model having different sizes and \ion{The previous paragraph argues for different size but not for different lyfe cycles} life cycles.
% Concretely, as shown in Figure~\ref{fig:contrast}, Hymba model contains three types of the KV caches, where the KV cache for self attention layers need to be always kept in GPU memory when this request is in the current batch of LLM inference engine, the KV cache of Mamba layer is much larger in size but only the KV cache of last token needs to be stored in GPU, and the KV cache of sliding windows layers have the same size per token as the self attention layers while need to save the last several tokens in GPU. However, PagedAttention can only allocate the same size of memory to tokens in different stages (a token outside sliding window / a token in sliding window / the last token)  of lifecycle due to its single page size design, and frees the memory of that token only when the life cycle of all layers ends, which causes severe memory waste.
% This also creates new GPU memory saving opportunity for GPU memory management system when it comes to prefix caching.
% For example, if one wants to cache the prefix of the prefix of the current request, it only needs to cache the KV cache for the last token in the prefix for Mamba layers, while for those self attention layers the KV cache for all  tokens need to be cached.

% \kt{Chen can you align the examples}
% \kt{Align the examples and draw figures.}
% \kt{Add more descriptions of the difficulty, and spell out concrete challenges, put prefix caching earlier}
% \kt{WE can be more kind to the reviewers --- heterogeneous memory states, a strawmen solution: static partitioning, obviously bad, dynamically multiplexing, }
% \kt{Chunked prefill -- probably not doable, preemption}

The breaking of these two assumptions can lead to $2.08\times$ throughput degredation in widely used heterogeneous LLMs in practice compared with an oracle implementation that handles the granularity and dependency rules perfectly. To address this problem, it is essential to re-design the GPU memory management system to maximize GPU memory utilization for heterogeneous LLMs, with varying KV cache sizes and dependency rules.

A straightforward approach to this problem is to statically partition the GPU memory into multiple fixed-size memory pools, each dedicated to a specific type of memory.\ps{Do you mean like slab memory allocation}
This method effectively handles different granularities between different attention layers.
However, static partitioning can have significant memory waste due to different dependency rules across different KV cache types. For example, while the total KV cache size of all tokens for a sliding window layer and a self-attention layer is the same for short requests that are smaller than the sliding window size, it differs a lot for requests with long contexts.




The problem of memory management for objects with varying sizes and dependency rules is challenging in general and has inspired decades of research~\tocite{}.
In LLM applications, however, this problem becomes more tractable. 
Despite the heterogeneity in granularities and dependencies inside LLMs, we find two empirical properties that apply to the majority of production-level LLMs:
\begin{itemize}
    \item \textbf{Large Granularity:} KV cache granularity in production-level LLMs is typically multipliers of \cred{$2^{12}$} bytes, \ps{this is interesting, is the number citable? or it will be explained in appendix? +1, is there any reason not to say 4KB?} which is essential for efficient parallelization by GPU kernels.
    This allows for splitting the memory into a \textit{\textbf{compatible size}} first, where different types of KV cache can perform memory allocation on top of this compatible size with little internal memory fragmentation, and then implement \textit{\textbf{customized memory allocators}} for different layers using such customized granularity. 
   \item \textbf{Prefix-Subset Dependency:} Due to the auto-regressive nature of LLMs, the KV cache dependencies in the same model generally follow a \textit{prefix-subset} dependency. 
   This means that the generation of a new token only requires a subset of its prefix tokens' KV cache. \ps{someone cannot understand. ``would be good to mention what is the context of this statement''}
   Based on this insight, we can provide \textbf{\textit{general support}} for prefix-subset dependency first, and then implement \textbf{\textit{customized logic}} for each attention variant to define the exact prefix subset required for new token generation.
\end{itemize}
% \zcsay{problem -> solution -> insight}
% \zcsay{some pages need to hit together, challenging to cache system}
% \zcsay{the importance of tokens of current request: the longer the important. the importance for future requests: this property not hold (e.g., system prompt, long context qa)}

% These two assumptions are not always true for all LLMs: people can use LLMs with, for example, a multiplier of 1000 bytes as the granularity, and the token dependency can be not only prefix but also suffix (e.g. bidirectional LLMs that can perform token infilling). That said, existing production-level LLMs all fall into this pattern. \kt{We probably need to fine-tune the wording here --- all sounds a little bit strong} \zcsay{we can remove this paragraph} \kt{We probably need this --- reviewers appreciate those papers that clearly states the limitation, and stating limitations do not weaken the paper (in fact it strengthens the paper)}

% We point out that two assumptions share the same pattern at a high level: there are some common functionalities shared by different attention layers in the LLM, while there are functionalities that needs to be customized based on the type of attention layer.  \zcsay{we can remove this paragraph and highlight compatable and customization before}

The compatible and customizable nature of these two properties motivates the design of a two-level GPU memory allocator, consisting of:
\begin{enumerate}
    \item A \textit{\textbf{compatible base memory manager}} that allocates memory using a page size compatible with different KV cache sizes inside the model and manages dependency with a general API.
    \item \textit{\textbf{Customizable managers}} for each type of memory that borrow and return memory from the base memory allocator, and executes customized allocation logic to handle the dependency of their respective KV caches. 
\end{enumerate}

To this end, we propose \sys, the first GPU memory allocator that maximizes GPU memory utilization for heterogeneous LLMs using traditional self-attention alongside other types of attention mechanisms:
(1) For the base memory manager, \sys uses the LCM of different KV cache sizes as the compatible size and provides an API to annotate the importance of allocated memory for better prefix caching and eviction design. \zcsay{should we admit it is a variant of slab allocator?}
(2) For customization managers, \sys leverages the API exposed by the base memory manager to customize the allocation, caching, and eviction logic for a wide range of attention layers (e.g., sliding window, Mamba, cross-attention). It accounts for different granularities and performs effective caching management by being aware of the dependency between tokens.

% To this end, we propose \sys, the first GPU memory allocator that maximizes GPU memory utilization for heterogeneous LLMs that uses traditional self-attention together with other types of attentions:
% (1) For the base memory manager, \sys uses the LCM of different KV cache sizes as the compatible size, and also exposes the API to annotate the importance of the allocated memory for better prefix caching and eviction design; (2) For customization managers, \sys leverages the API exposed by base memory manager to customize the allocation, caching and eviction logic for a wide range of attention layers (e.g., sliding window, mamba, cross attention), in a way that is aware of different granularities, and do effective caching management by being awaring of the dependency between tokens.

To make \sys practical, we further make it work with a wide range of LLM inference engine optimizations (e.g. speculative decoding and chunked prefill) and features (e.g., multi-modality inputs).
% the prefix caching feature of existing LLM inference engines, while making sure that the prefix cache eviction is fair for different types of KV caches. \zcsay{does the discussions before this paragraph include prefix caching? I think including prefix caching like this is quite strange}

% The practical challenge of \sys is: how to support the widely-used prefix caching optimization, so that the KV caches computed by one request can be reused by another request with the same prefix?
% To handle this challenge, we engineer the allocation, caching and eviction logic for a wide range of attention layers, so that it is compatible with the prefix caching feature of existing LLM inference engines, while making sure that the prefix cache eviction is fair for different types of KV caches. \zcsay{does the discussions before this paragraph include prefix caching? I think including prefix caching like this is quite strange}

We evaluate \sys on seven LLMs, three datasets, and two types of GPUs. Compared with vLLM, the state-of-the-art LLM serving engine, \sys achieves \cred{1.85}$\times$  higher throughput on average (up to 4.92$\times$)  without hurting the end-to-end latency, by maximally batching LLM inference requests with little memory waste.\ps{quantify this}

The contribution of this paper is as follows:
\begin{itemize}
    \item We identify the heterogeneous LLM senerio, a new trend for frontier model structures.
    \item We propose a two-level design for LLM memory management system. This includes a compatible level for coordinating different types of layers within a model, and a customizable level for addressing the unique properties of each layer type.
    \item A practical implementation, \sys, that is built on top of production-level inference engine vLLM and is compatible to a wide range of inference engine features.
    \item \sys achieves a \cred{1.85}$\times$ improvement in serving throughput without sacrificing request serving latency.
\end{itemize}

% \item Practical problems
%     \begin{itemize}
%         \item Memory allocation: how to avoid internal fragmentation in large page
%         \item Accelerators like GPUs needs regular pages (with only one page size) to execute efficiently, but we have multiple page sizes now
%         \item Allow each type to customize cache management strategy flexibly % Cache replacement policies. ) 2. fair replacement policies for different types
%     \end{itemize}
% \item Solutions
%     \begin{itemize}
%         \item Memory allocation: request-aware allocation to avoid internal fragmentation
%         \item Execution: represent the allocation result of each layer as single-size pages, with minimal changes to the workers
%         \item Cache replace policy: flexible interface to custom last access time of different types of pages %, unified LRU for fair replacement
%     \end{itemize}
% \end{itemize}

% \zc{show new eviction policy as our contribution}

% \kt{
% 7. Two functionalities: 1. which memory need to be allocated (allocation) 2. what should be the type of that allocated memory (instantiation)
% We argue that, we should decouple these two dec
% which memory need to be allocated to what type.
% We argue that we should implement \textit{multiple} memory allocators to allow the allocation / free of different types to decouple with other types, while these multiple memory allocators need 
% }


% 1) which memory should be allocated to which type
% 2) how to use this piece of memory

% how to customize the allocate / \cred{access, need replace} /free patterns of the heterogeneous types, while allowing these customized memory access patterns compatible with each other

% how to customized the usage of memory of hetergeneous type, while allowing these things to exchange memory with each other as needed.

% \item We argue for a \textit{two-layer} desi

% \item Insight: we design a new that can be repurposed 
% \item then, two questions: 1) how to express the unique memory patterns of different component 2) how to fairly and efficiently distributed the overall memory resource to different types

% \subsection{12/03 Woosuk}

% \zcsay{
% \begin{enumerate}
%     \item follow Ion's flow on pointing the two assumptions in PagedAttention explicitly and then show the problem
%     \item Better to say "PagedAttention assumed all the prefix is required to generate next tokens" rather than "different KV caches have different lifecycles" since "lifecycle" is a bit vague 
%     \item remove life cycle and discuss dependency directly
%     \item move vAttention to related work, introduce dependency when pointing out the problem
%     \item show more relationship to the insight when introducing the solution
%     \item polish the text and then discuss about how to compress it
%     \item talk more about design in the summarization of contribution, talk less about performance improvement
% \end{enumerate}
% }
% The key reason behind such inefficiency is that a single LLM request cannot fully saturate the GPU's parallel computing capability, since LLMs are auto-regressive models that have to generate tokens one-by-one. 

% \zcsay{prefer to simplify this paragraph, just mention it is expensive in one sentence} \kt{I am already reducing the points compared to Ion's outline. Shall we keep simplifying it?}

% Such massive batching challenges the GPU memory management system design, as the KV cache, the intermediate tensors generated by LLM's attention module that can be large, of all requests in the batch needs to be stored on GPU in order to perform batched inference.
% PagedAttention provides a practical solution for those LLMs that only use self-attention attention mechanism, which is a valid assumption for early-stage LLMs.

% PagedAttention~\tocite{} is a widely-adopted acceleration technique for LLM inference.
% \kt{Need some number to let reviewer know that these two types of models are REALLY popular}


% : more and more LLMs customize the attention layers in order to fit specific user needs and breaks the two assumptions.


% GPU memory management systems for those LLMs that only use self-attention attention mechanism, which is a valid as-
% sumption for early-stage LLMs.


% provides a practical implementation of GPU memory management systems for those LLMs that only use self-attention attention mechanism, which is a valid assumption for early-stage LLMs.

% To accelerate LLM inference, there are two widely-adopted optimizations:
% \begin{itemize}
% \item \textit{Continuous batching}: Currently-running LLM LLM inference requests can be batched together with new incoming requests to saturate GPU's parallel computing capability. 
% \item \textit{Prefix caching}: One can cache the KV Cache (the intermediate tensors generated by LLM's attention layers) of the current request for future use: if a future request share the same prefix with the current request, the KV caches correspond to that prefix can be reused to save GPU computation. 
% \end{itemize}
% Both optimizations challenge GPU memory management systems. 
% Continuous batching requires the memory allocation to lower the GPU memory fragmentation, so that the KV cache of more requests can be kept in GPU and the batch size can be larger.
% Prefix caching requires the GPU memory system to store the KV cache of as many frequently-reused prefixes as possible and evict the KV caches when more GPU memory is requires to finish processing the current batch of LLM inference requests.
% \zc{simplify this paragraph}

% evict those infrequenly-reused prefixes out from the GPU memory.

% Both of these two techniques challenge the design of GPU memory management system.
% Continuous batching requires the GPU memory management system to store the KV cache of as many requests into GPU as possible to maximally increase the batch size, highlighting the need to an efficient memory allocation module that can allocate GPU memory space of KV caches with low GPU memory fragmentation.
% Prefix caching requires the GPU memory management system to trade between caching the KV caches of one request (so that it can be reused for future request) or discarding the KV cache (to free GPU memory), which requires the GPU memory management to keep frequently-reused KV caches into GPU memory and evict other KV caches from the GPU.

% Another solution is to utilize GPU driver to dynamically allocate pages like vAttention. However, the GPU driver is agnostic to the dependency between tokens inside KV caches. For self attention layers, a token can be cache hitted only when both it and all its prefix tokens exist in the cache, and for sliding window layers, a token can be cache hitted only when there are at least sliding window size consecutive tokens in the cache. However, GPU drivers can not manage the cache automiatically without breaking such dependency due to its agnostic to applications. \zcsay{discuss dependency earlier, and move to related work}

% \zcsay{should make the concept ``GPU driver'' broader. e.g., general os memory management also cannot handle it}
% \woosuk{I think we don't need to mention vAttention here. Hurts the story.}

% One potential solution for this problem is to statically partition the GPU memory into multiple fix-size memory pools, and handle different types of KV caches inside different memory pools.
% Such solution works well when the KV cache size ratio between differnet types of attention layers is relatively fixed.
% However, this assumption does not hold for \mamba.
% This is because that, for self attention layers the KV cache of \textit{all} tokens need to be kept in GPU, but for Mamba layers only the KV cache of \textit{the last} token need to be kept in GPU.
% As a result, the size ratio between self-attention KV caches and Mamba KV caches hugely varies when the request lengths are different.
% In this scenario, such static partition strategy will result in high GPU memory fragmentation. \zcsay{prefer sliding window here. if not considering prefix caching, fix size partition works well for mamba as mamba cache is very very small.}


% Another potential solution is vAttention, where it tailors the GPU memory allocator inside the GPU driver to allocate KV caches with minimum fragmentation.
% However, the GPU driver is agnostic to the dependency between KV caches, where we say that KV Cache A depends on KV Cache B, if the KV cache A cannot be reused unless KV cache B is also stored in GPU memory.
% For example, as the self attention KV cache of all tokens in the prefix need to be stored in GPU in order to reuse this prefix, the KV cache of all other tokens all depends on the KV cache of the first token. 
% If we evict the KV cache of the first token, even if we store the KV cache of all other tokens, that KV cache cannot be reused.
% Since such dependency is not visible in the GPU driver, it will wrongfully evict the KV caches that other KV caches depend on, and the other KV caches becomes useless to store in GPU. \zcsay{we can use some figure to explain it}

% To conclude, when handling heterogeneous LLMs, previous work either have high GPU memory fragmentation, or waste GPU memory to store KV caches that cannot be reused by prefix caching.

    % \item The number of different types of KV caches is relatively limited: at most five different types KV caches need to be stored in GPU when serving a LLM. \kt{This argument does not directly motivate the compatibility itself, instead it argues that if we do compatible layer, the overhead is small. So it is probably not a good argument for here.} \cred{VOTE: should we keep this point?}

        % and it allows the GPU memory freed by one types of KV caches can be reused by another.
    % \zc{KV cache sizes inside the same LLM are typically a multiplier of \cred{$2^{10}$} bytes due to the parallelization requirement of GPU architecture. The highly-aligned KV cache size makes compatible page size possible}

       % though different types of KV cache can have hugely-different life cycles and dependency rules, they can be fully determined based on pre-known model configurations like sliding window size without more runtime information. 
   % As a result, we can provide interface and implementations for different types of KV caches to \textit{customize} their life cycles, and their dependency rule between tokens. 
   % \zcsay{I prefer textit ``customize'' instead of ``dependency''. I change the meaning of this insight. Kuntai you can revert if you are not comfortable.}
   % \cred{Current best answer: different types of KV caches all need to customize their prefix caching policy based on the workload to achieve best performance.}
   % \cred{A weaker argument: some KV caches no longer need to be stored in GPU if its dependent KV caches are evicted }

